Automated Deep Neural Network Inference Partitioning for Distributed Embedded Systems

Distributed systems can be found in various applications, e.g., in robotics or autonomous driving, to achieve higher flexibility and robustness. Thereby, data flow centric applications such as Deep Neural Network (DNN) inference benefit from partitioning the workload over multiple compute nodes in terms of performance and energy-efficiency. However, mapping large models on distributed embedded systems is a complex task, due to low latency and high throughput requirements combined with strict energy and memory constraints. In this paper, we present a novel approach for hardware-aware layer scheduling of DNN inference in distributed embedded systems. Therefore, our proposed framework uses a graph-based algorithm to automatically find beneficial partitioning points in a given DNN. Each of these is evaluated based on several essential system metrics such as accuracy and memory utilization, while considering the respective system constraints. We demonstrate our approach in terms of the impact of inference partitioning on various performance metrics of six different DNNs. As an example, we can achieve a 47.5 % throughput increase for EfficientNet-B0 inference partitioned onto two platforms while observing high energy-efficiency.

==> figures/eval_alexnet_result.tex <==
0,0,/features/features.2/MaxPool,1,2,14.556510000000003,3.5950940473719992,87.47804301120418,93312.0,424640.0,61347200.0,nondom
1,0,/features/features.5/MaxPool,1,2,19.282429999999998,4.738269248692995,85.49463777631868,64896.0,731840.0,60889856.0,nondom
2,0,output,1,2,23.278478,4.9632504174496,42.9588694600242,0.0,61491904.0,0.0,sensor
3,0,/features/features.1/Relu,1,2,17.063918,5.099538847371999,87.47804301120418,401408.0,424640.0,61347200.0,dom
4,0,/features/features.4/Relu,1,2,21.032494,5.788307648692995,85.49463777631868,279936.0,731840.0,60889856.0,dom
5,0,/features/features.6/Conv,1,2,21.214541999999998,5.227136299652277,65.39845973547632,129792.0,1395392.0,60204672.0,dom
6,0,/features/features.9/Relu,1,2,22.734398,5.2376062180548955,49.79286169534736,86528.0,2280128.0,59298304.0,dom
7,0,/features/features.10/Conv,1,2,23.982398,5.3856024174496,42.9588694600242,86528.0,2869952.0,58674432.0,dom
8,0,/avgpool/AveragePool,1,2,23.428269999999998,5.0531256174495995,42.9588694600242,18432.0,2869952.0,58635264.0,dom
9,0,/classifier/classifier.2/Relu,1,2,23.344894,5.0031000174496,42.9588694600242,8192.0,40618688.0,20881408.0,dom
10,0,/classifier/classifier.4/Gemm,1,2,23.344894,5.0031000174496,42.9588694600242,8192.0,57395904.0,4101096.0,dom
11,0,/classifier/classifier.6/Gemm,1,2,23.294525999999998,4.9728792174495995,42.9588694600242,2000.0,61491904.0,1000.0,dom
12,0,input,1,2,15.845198,4.552279467762434,75.0259589818077,309174.0,154587.0,61491904.0,edge
13,0,/features/features.0/Conv,1,2,17.063918,5.099538847371999,87.47804301120418,401408.0,378523.0,61347200.0,dom
14,0,/features/features.7/Relu,1,2,21.214541999999998,5.227136299652277,65.39845973547632,129792.0,1395392.0,60183040.0,dom
15,0,/features/features.8/Conv,1,2,22.734398,5.2376062180548955,49.79286169534736,86528.0,2280128.0,59298304.0,dom
16,0,/Flatten,1,2,23.428269999999998,5.0531256174495995,42.9588694600242,18432.0,2869952.0,58630144.0,dom
17,0,/classifier/classifier.1/Gemm,1,2,23.344894,5.0031000174496,42.9588694600242,8192.0,40618688.0,20881408.0,dom
18,0,/classifier/classifier.5/Relu,1,2,23.344894,5.0031000174496,42.9588694600242,8192.0,57395904.0,4098000.0,dom


==> figures/eval_efficientnet_result.tex <==
0,0,input,1,2,308.937616,87.6210838927631,3.2627776162884126,301056.0,150528.0,166675168.0,edge
1,0,/features/features.0/features.0.,1,2,312.779456,90.11376295631237,3.268797999234121,802816.0,552800.0,166674304.0,nondom
2,0,/features/features.1/features.1.,1,2,313.65199800000005,88.59651654228264,3.2944643642401967,401408.0,1215328.0,166664064.0,nondom
3,0,/features/features.2/features.2.,1,2,317.523646,88.93329400759919,3.3563613284075378,301056.0,3711328.0,164318592.0,nondom
4,0,/features/features.2/features.2.,1,2,321.56719200000003,89.68157955616964,3.5443874270653675,150528.0,3906592.0,164123328.0,nondom
5,0,/features/features.3/features.3.,1,2,327.786808,93.3965558638178,3.547936669046622,903168.0,3910048.0,163360960.0,nondom
6,0,/features/features.3/features.3.,1,2,327.90160199999997,91.78539905971799,3.6876444219842317,125440.0,4435936.0,162803712.0,nondom
7,0,/features/features.3/features.3.,1,2,331.12117,93.64190562419869,3.6897779351427067,501760.0,4445536.0,162794112.0,nondom
8,0,/features/features.3/features.3.,1,2,352.694776,97.74025498448131,4.019098434231593,62720.0,5899936.0,161339712.0,nondom
9,0,/features/features.4/features.4.,1,2,353.92964600000005,97.47315521976768,4.055199044984403,62720.0,6451936.0,160640320.0,nondom
10,0,/features/features.4/features.4.,1,2,355.538134,98.41796043753034,4.057617848844158,250880.0,6490336.0,160601920.0,nondom
11,0,/features/features.4/features.4.,1,2,358.243646,96.26391983433113,4.195253473439136,62720.0,8621536.0,158470720.0,nondom
12,0,/features/features.4/features.4.,1,2,359.85213400000004,97.2087250520938,4.197842292270403,250880.0,8659936.0,158432320.0,nondom
13,0,/features/features.4/features.4.,1,2,362.3023980000001,94.90153564889458,4.345328090086645,31360.0,10791136.0,156301120.0,nondom
14,0,/features/features.5/features.5.,1,2,363.65563800000007,95.69319206665723,4.348105499996911,188160.0,10829536.0,156262720.0,nondom
15,0,/features/features.5/features.5.,1,2,381.21868600000005,91.46442500592714,4.8139638842950285,87808.0,16662496.0,150429760.0,opt
16,0,/features/features.5/features.5.,1,2,383.7331260000001,92.79270164300124,4.820650122516821,351232.0,16737760.0,150354496.0,nondom
17,0,/features/features.6/features.6.,1,2,542.3666420000001,112.37175210136016,1.8874191472104265,18816.0,152341216.0,14522112.0,nondom
18,0,output,1,2,548.9520980000001,114.37373444961958,1.8216538904971054,0.0,166675168.0,0.0,sensor
19,0,/features/features.0/features.0.,1,2,319.313264,94.03404775631238,3.268797999234121,1605632.0,803680.0,166674304.0,dom
20,0,/features/features.0/features.0.,1,2,312.779456,90.11376295631237,3.268797999234121,802816.0,1205088.0,166674304.0,dom
21,0,/features/features.1/features.1.,1,2,323.07646400000004,94.43116539555905,3.293103355728302,1605632.0,1214304.0,166665088.0,dom
22,0,/features/features.1/features.1.,1,2,316.54316800000004,90.51118779555905,3.293103355728302,802880.0,1214304.0,166665088.0,dom
23,0,/features/features.1/features.1.,1,2,316.54368000000005,90.51149499555905,3.293103355728302,802944.0,1214304.0,166665088.0,dom
24,0,/features/features.1/features.1.,1,2,316.543439,90.51135370852391,3.2931034099509517,802912.0,1214560.0,166664832.0,dom
25,0,/features/features.1/features.1.,1,2,316.54331099999996,90.51127690852391,3.2931034099509517,802896.0,1214560.0,166664832.0,dom
26,0,/features/features.1/features.1.,1,2,316.543198,90.51121238253893,3.293103464173603,802880.0,1214816.0,166664576.0,dom
27,0,/features/features.1/features.1.,1,2,316.543198,90.51121238253893,3.293103464173603,802880.0,1214816.0,166664576.0,dom
28,0,/features/features.2/features.2.,1,2,324.764366,93.32018346305827,3.354772116368725,1204224.0,3708256.0,164396928.0,dom
29,0,/features/features.2/features.2.,1,2,319.865598,90.38092266305827,3.354772116368725,602304.0,3708256.0,164396928.0,dom
30,0,/features/features.2/features.2.,1,2,319.86713399999996,90.38184426305827,3.354772116368725,602496.0,3708256.0,164396928.0,dom
31,0,/features/features.2/features.2.,1,2,319.865756,90.38102801339515,3.354772228913688,602320.0,3708640.0,164396544.0,dom
32,0,/features/features.2/features.2.,1,2,319.86569199999997,90.38098961339514,3.354772228913688,602312.0,3708640.0,164396544.0,dom
33,0,/features/features.2/features.2.,1,2,319.86567799999995,90.38097968134345,3.354772341458659,602304.0,3709024.0,164396160.0,dom
34,0,/features/features.2/features.2.,1,2,319.86567799999995,90.38097968134345,3.354772341458659,602304.0,3709024.0,164396160.0,dom
35,0,/features/features.2/features.2.,1,2,332.31884599999995,97.79362071524733,3.3595438223263594,2107392.0,3714784.0,164315136.0,dom
36,0,/features/features.2/features.2.,1,2,337.399166,99.16598807257293,3.540844526828094,2107392.0,3901408.0,164128512.0,dom
37,0,/features/features.2/features.2.,1,2,330.051118,94.75715927257293,3.540844526828094,1204512.0,3901408.0,164128512.0,dom
38,0,/features/features.2/features.2.,1,2,322.79221600000005,90.41659395616963,3.5443874270653675,301056.0,3906592.0,164123328.0,dom
39,0,/features/features.3/features.3.,1,2,327.786808,93.3965558638178,3.547936669046622,903168.0,3910048.0,163668288.0,dom
40,0,/features/features.3/features.3.,1,2,335.13736800000004,97.80689186381778,3.547936669046622,1806336.0,3910048.0,163360960.0,dom
41,0,/features/features.3/features.3.,1,2,330.46192799999994,93.3696794475867,3.6863646826209586,451584.0,4428448.0,162842560.0,dom
42,0,/features/features.3/features.3.,1,2,328.62671,92.26858854403544,3.6863650902995406,226104.0,4429312.0,162841696.0,dom
43,0,/features/features.3/features.3.,1,2,328.62661399999996,92.26853094403545,3.6863650902995406,226092.0,4429312.0,162841696.0,dom
44,0,/features/features.3/features.3.,1,2,328.626578,92.26852884273463,3.686365497978213,226080.0,4430176.0,162840832.0,dom
45,0,/features/features.3/features.3.,1,2,359.173938,101.67050154178303,4.016563988563718,878080.0,5885536.0,161354112.0,dom
46,0,/features/features.3/features.3.,1,2,356.11501,99.83514474178303,4.016563988563718,502240.0,5885536.0,161354112.0,dom
47,0,/features/features.3/features.3.,1,2,356.119058,99.83757354178303,4.016563988563718,502720.0,5885536.0,161354112.0,dom
48,0,/features/features.3/features.3.,1,2,356.11535,99.83548145766461,4.016565601842993,502280.0,5887936.0,161351712.0,dom
49,0,/features/features.3/features.3.,1,2,356.11519,99.83538545766461,4.016565601842993,502260.0,5887936.0,161351712.0,dom
50,0,/features/features.3/features.3.,1,2,356.11508,99.8354411926062,4.0165672151235645,502240.0,5890336.0,161349312.0,dom
51,0,/features/features.3/features.3.,1,2,356.11508,99.8354411926062,4.0165672151235645,502240.0,5890336.0,161349312.0,dom
52,0,/features/features.3/features.3.,1,2,353.20527200000004,98.0465525844813,4.019098434231593,125440.0,5899936.0,161339712.0,dom
53,0,/features/features.4/features.4.,1,2,358.466616,101.12812474896202,4.021632845672816,752640.0,5909536.0,161182720.0,dom
54,0,/features/features.4/features.4.,1,2,355.403848,99.29046394896201,4.021632845672816,376320.0,5909536.0,161182720.0,dom
55,0,/features/features.4/features.4.,1,2,354.9120680000001,98.07415698557385,4.053987437179409,188160.0,6427936.0,160664320.0,dom
56,0,/features/features.4/features.4.,1,2,354.15037200000006,97.61713938557385,4.053987437179409,94560.0,6427936.0,160664320.0,dom
57,0,/features/features.4/features.4.,1,2,354.15421200000003,97.61944338557385,4.053987437179409,95040.0,6427936.0,160664320.0,dom
58,0,/features/features.4/features.4.,1,2,354.15071200000006,97.61747610145544,4.0539890806614896,94600.0,6430336.0,160661920.0,dom
59,0,/features/features.4/features.4.,1,2,354.15055200000006,97.61738010145544,4.0539890806614896,94580.0,6430336.0,160661920.0,dom
60,0,/features/features.4/features.4.,1,2,354.15044200000006,97.61743583639702,4.053990724144903,94560.0,6432736.0,160659520.0,dom
61,0,/features/features.4/features.4.,1,2,354.15044200000006,97.61743583639702,4.053990724144903,94560.0,6432736.0,160659520.0,dom
62,0,/features/features.4/features.4.,1,2,361.22741400000007,98.06933758293191,4.192660814327092,439040.0,8563936.0,158528320.0,dom
63,0,/features/features.4/features.4.,1,2,358.243646,96.26391983433113,4.195253473439136,62720.0,8621536.0,158470720.0,dom
64,0,/features/features.4/features.4.,1,2,364.01781400000004,95.94594219749536,4.342546683028223,251840.0,10733536.0,156358720.0,dom
65,0,/features/features.4/features.4.,1,2,362.5576460000001,95.05468444889458,4.345328090086645,62720.0,10791136.0,156301120.0,dom
66,0,/features/features.5/features.5.,1,2,365.18691800000005,96.61196006665723,4.348105499996911,376320.0,10829536.0,156262720.0,dom
67,0,/features/features.5/features.5.,1,2,381.93352600000003,91.93057478613332,4.809190092952987,189120.0,16589536.0,150502720.0,dom
68,0,/features/features.5/features.5.,1,2,381.935966,91.93152707608633,4.809194718619306,189200.0,16599136.0,150493120.0,dom
69,0,/features/features.5/features.5.,1,2,381.935646,91.93133507608633,4.809194718619306,189160.0,16599136.0,150493120.0,dom
70,0,/features/features.5/features.5.,1,2,381.9355260000001,91.93171569954751,4.809199344294522,189120.0,16608736.0,150483520.0,dom
71,0,/features/features.5/features.5.,1,2,381.9355260000001,91.93171569954751,4.809199344294522,189120.0,16608736.0,150483520.0,dom
72,0,/features/features.5/features.5.,1,2,421.6861180000001,97.22828816548997,3.9610131732999507,614656.0,28027360.0,139064896.0,dom
73,0,/features/features.5/features.5.,1,2,419.55328600000007,95.94858896548996,3.9610131732999507,352576.0,28027360.0,139064896.0,dom
74,0,/features/features.5/features.5.,1,2,419.55432200000007,95.95022059354743,3.961004387129239,352688.0,28046176.0,139046080.0,dom
75,0,/features/features.5/features.5.,1,2,458.01695800000005,100.4636629081145,3.006735870100351,614656.0,39505120.0,127565184.0,dom
76,0,/features/features.5/features.5.,1,2,455.89487800000006,99.1904149081145,3.006735870100351,353920.0,39505120.0,127565184.0,dom
77,0,/features/features.5/features.5.,1,2,455.8851620000001,99.18559533617196,3.006730807450943,352688.0,39523936.0,127546368.0,dom
78,0,/features/features.5/features.5.,1,2,455.8847140000001,99.18532653617196,3.006730807450943,352632.0,39523936.0,127546368.0,dom
79,0,/features/features.5/features.5.,1,2,455.8844060000001,99.1861567582925,3.0067257448185845,352576.0,39542752.0,127527552.0,dom
80,0,/features/features.5/features.5.,1,2,455.8844060000001,99.1861567582925,3.0067257448185845,352576.0,39542752.0,127527552.0,dom
81,0,/features/features.6/features.6.,1,2,455.68007000000006,98.83460952825027,2.9968356412464074,263424.0,39693280.0,127245312.0,dom
82,0,/features/features.6/features.6.,1,2,463.56037000000003,99.83363653924445,2.829317729834674,131712.0,50982880.0,115880448.0,dom
83,0,/features/features.6/features.6.,1,2,463.03533000000004,99.51861253924444,2.829317729834674,67200.0,50982880.0,115880448.0,dom
84,0,/features/features.6/features.6.,1,2,463.0462900000001,99.52518853924445,2.829317729834674,68544.0,50982880.0,115880448.0,dom
85,0,/features/features.6/features.6.,1,2,463.0363660000001,99.5202441673019,2.8293132470200395,67312.0,51001696.0,115861632.0,dom
86,0,/features/features.6/features.6.,1,2,463.0359180000001,99.5199753673019,2.8293132470200395,67256.0,51001696.0,115861632.0,dom
87,0,/features/features.6/features.6.,1,2,463.0356100000001,99.52080558942244,2.8293087642196104,67200.0,51020512.0,115842816.0,dom
88,0,/features/features.6/features.6.,1,2,463.0356100000001,99.52080558942244,2.8293087642196104,67200.0,51020512.0,115842816.0,dom
89,0,/features/features.6/features.6.,1,2,490.21688200000006,104.26765300900416,2.4270976324779054,152832.0,84548320.0,82315008.0,dom
90,0,/features/features.6/features.6.,1,2,490.2357300000001,104.27896180900416,2.4270976324779054,155136.0,84548320.0,82315008.0,dom
91,0,/features/features.6/features.6.,1,2,516.770242,108.62179115454701,2.1242895472930794,152832.0,118278880.0,48584448.0,dom
92,0,/features/features.6/features.6.,1,2,544.22373,113.51600610008984,1.8886579479920262,263424.0,152009440.0,14853888.0,dom
93,0,/features/features.6/features.6.,1,2,543.347306,112.98011842348609,1.8885757672235182,153024.0,152064736.0,14798592.0,dom
94,0,/features/features.6/features.6.,1,2,543.3463300000001,112.9795328234861,1.8885757672235182,152928.0,152064736.0,14798592.0,dom
95,0,/features/features.6/features.6.,1,2,543.3464020000001,112.98222383866309,1.8885689191489667,152832.0,152120032.0,14743296.0,dom
96,0,/features/features.6/features.6.,1,2,543.3464020000001,112.98222383866309,1.8885689191489667,152832.0,152120032.0,14743296.0,dom
97,0,/features/features.6/features.6.,1,2,542.5198740000001,112.46369130136016,1.8874191472104265,37632.0,152341216.0,14522112.0,dom
98,0,/features/features.7/features.7.,1,2,549.2682739999999,114.75717802767133,1.8262678014997387,117504.0,164506336.0,2356992.0,dom
99,0,/features/features.7/features.7.,1,2,549.272922,114.74993355106758,1.8261909604789266,115392.0,164561632.0,2301696.0,dom
100,0,/features/features.7/features.7.,1,2,549.272154,114.74947275106759,1.8261909604789266,115296.0,164561632.0,2301696.0,dom
101,0,/features/features.7/features.7.,1,2,549.272226,114.75216376624456,1.8261845573524034,115200.0,164616928.0,2246400.0,dom
102,0,/features/features.7/features.7.,1,2,549.272226,114.75216376624456,1.8261845573524034,115200.0,164616928.0,2246400.0,dom
103,0,/features/features.8/features.8.,1,2,549.9727220000001,114.98610884961957,1.8216538904971054,125440.0,165395168.0,1405440.0,dom
104,0,/features/features.8/features.8.,1,2,550.9937140000001,115.59870404961957,1.8216538904971054,250880.0,165395168.0,1344000.0,dom
105,0,/features/features.8/features.8.,1,2,549.9727220000001,114.98610884961957,1.8216538904971054,125440.0,165395168.0,1282560.0,dom
106,0,/avgpool/GlobalAveragePool,1,2,548.9726260000001,114.38605124961957,1.8216538904971054,2560.0,165395168.0,1282280.0,dom
107,0,/features/features.1/features.1.,1,2,316.542656,90.51088059555906,3.293103355728302,802816.0,1214304.0,166665088.0,dom
108,0,/features/features.1/features.1.,1,2,316.54331099999996,90.51127690852391,3.2931034099509517,802896.0,1214560.0,166664832.0,dom
109,0,/features/features.1/features.1.,1,2,316.542686,90.51090518253892,3.293103464173603,802816.0,1214816.0,166664576.0,dom
110,0,/features/features.2/features.2.,1,2,330.613822,98.51611379552975,3.2985538216450836,2408448.0,1417568.0,165458304.0,dom
111,0,/features/features.2/features.2.,1,2,350.215454,110.27709299552974,3.2985538216450836,4816896.0,2421088.0,164555136.0,dom
112,0,/features/features.2/features.2.,1,2,330.613822,98.51611379552975,3.2985538216450836,2408448.0,3625312.0,164479872.0,dom
113,0,/features/features.2/features.2.,1,2,319.864062,90.38000106305827,3.354772116368725,602112.0,3708256.0,164396928.0,dom
114,0,/features/features.2/features.2.,1,2,319.86569199999997,90.38098961339514,3.354772228913688,602312.0,3708640.0,164396544.0,dom
115,0,/features/features.2/features.2.,1,2,319.86414199999996,90.38005808134345,3.354772341458659,602112.0,3709024.0,164396160.0,dom
116,0,/features/features.2/features.2.,1,2,324.968286,93.38328471524733,3.3595438223263594,1204224.0,3714784.0,164315136.0,dom
117,0,/features/features.2/features.2.,1,2,330.048606,94.75565207257294,3.540844526828094,1204224.0,3901408.0,164128512.0,dom
118,0,/features/features.2/features.2.,1,2,330.051244,94.75727476902168,3.5408449029555324,1204524.0,3902272.0,164127648.0,dom
119,0,/features/features.2/features.2.,1,2,328.82367200000004,94.02075106772087,3.540845279083051,1053696.0,3903136.0,164126784.0,dom
120,0,/features/features.3/features.3.,1,2,328.62418399999996,92.2670330475867,3.6863646826209586,225792.0,4428448.0,162842560.0,dom
121,0,/features/features.3/features.3.,1,2,328.62661399999996,92.26853094403545,3.6863650902995406,226092.0,4429312.0,162841696.0,dom
122,0,/features/features.3/features.3.,1,2,328.626578,92.26852884273463,3.686365497978213,226080.0,4430176.0,162840832.0,dom
123,0,/features/features.3/features.3.,1,2,356.11117,99.83284074178303,4.016563988563718,501760.0,5885536.0,161354112.0,dom
124,0,/features/features.3/features.3.,1,2,356.11519,99.83538545766461,4.016565601842993,502260.0,5887936.0,161351712.0,dom
125,0,/features/features.3/features.3.,1,2,355.60074399999996,99.52683959260621,4.0165672151235645,439040.0,5890336.0,161349312.0,dom
126,0,/features/features.4/features.4.,1,2,355.403848,99.29046394896201,4.021632845672816,376320.0,5909536.0,161182720.0,dom
127,0,/features/features.4/features.4.,1,2,354.14632400000005,97.61471058557385,4.053987437179409,94080.0,6427936.0,160664320.0,dom
128,0,/features/features.4/features.4.,1,2,354.15055200000006,97.61738010145544,4.0539890806614896,94580.0,6430336.0,160661920.0,dom
129,0,/features/features.4/features.4.,1,2,354.14639400000004,97.61500703639703,4.053990724144903,94080.0,6432736.0,160659520.0,dom
130,0,/features/features.4/features.4.,1,2,359.69613400000003,97.15056958293191,4.192660814327092,250880.0,8563936.0,158528320.0,dom
131,0,/features/features.4/features.4.,1,2,359.70593400000007,97.15593787288489,4.192664330010981,251880.0,8573536.0,158518720.0,dom
132,0,/features/features.4/features.4.,1,2,359.44288600000004,96.99856169634609,4.192667845700766,219520.0,8583136.0,158509120.0,dom
133,0,/features/features.4/features.4.,1,2,364.0101340000001,95.94133419749535,4.342546683028223,250880.0,10733536.0,156358720.0,dom
134,0,/features/features.4/features.4.,1,2,364.0199340000001,95.94670248744833,4.342550454573837,251880.0,10743136.0,156349120.0,dom
135,0,/features/features.4/features.4.,1,2,363.7568860000001,95.78932631090953,4.342554226126003,219520.0,10752736.0,156339520.0,dom
136,0,/features/features.5/features.5.,1,2,381.92563800000005,91.92584198613332,4.809190092952987,188160.0,16589536.0,150502720.0,dom
137,0,/features/features.5/features.5.,1,2,381.935646,91.93133507608633,4.809194718619306,189160.0,16599136.0,150493120.0,dom
138,0,/features/features.5/features.5.,1,2,381.9276380000001,91.92698289954751,4.809199344294522,188160.0,16608736.0,150483520.0,dom
139,0,/features/features.5/features.5.,1,2,419.54232600000006,95.94201296548997,3.9610131732999507,351232.0,28027360.0,139064896.0,dom
140,0,/features/features.5/features.5.,1,2,419.55387400000006,95.94995179354743,3.961004387129239,352632.0,28046176.0,139046080.0,dom
141,0,/features/features.5/features.5.,1,2,419.18513400000006,95.72972281566797,3.960995600997505,307328.0,28064992.0,139027264.0,dom
142,0,/features/features.5/features.5.,1,2,417.54952600000007,94.69979974855165,3.9541192472211035,87808.0,28140256.0,138930048.0,dom
143,0,/features/features.5/features.5.,1,2,420.06396600000005,96.02807638562575,3.9438493657777514,351232.0,28215520.0,138854784.0,dom
144,0,/features/features.5/features.5.,1,2,455.8731660000001,99.1773877081145,3.006735870100351,351232.0,39505120.0,127565184.0,dom
145,0,/features/features.5/features.5.,1,2,455.8847140000001,99.18532653617196,3.006730807450943,352632.0,39523936.0,127546368.0,dom
146,0,/features/features.5/features.5.,1,2,455.515974,98.96509755829248,3.0067257448185845,307328.0,39542752.0,127527552.0,dom
147,0,/features/features.5/features.5.,1,2,453.5231020000001,97.72081609117618,3.0027618803222826,43904.0,39618016.0,127452288.0,dom
148,0,/features/features.6/features.6.,1,2,455.68007000000006,98.83460952825027,2.9968356412464074,263424.0,39693280.0,127170048.0,dom
149,0,/features/features.6/features.6.,1,2,463.0243700000001,99.51203653924445,2.829317729834674,65856.0,50982880.0,115880448.0,dom
150,0,/features/features.6/features.6.,1,2,463.0359180000001,99.5199753673019,2.8293132470200395,67256.0,51001696.0,115861632.0,dom
151,0,/features/features.6/features.6.,1,2,463.02465000000007,99.51422958942244,2.8293087642196104,65856.0,51020512.0,115842816.0,dom
152,0,/features/features.6/features.6.,1,2,462.8597940000001,99.40127686473163,2.827803347089842,37632.0,51149536.0,115713792.0,dom
153,0,/features/features.6/features.6.,1,2,463.88944200000003,100.01270921083736,2.825226355723007,150528.0,51370720.0,115492608.0,dom
154,0,/features/features.6/features.6.,1,2,490.19824200000005,104.25646900900416,2.4270976324779054,150528.0,84548320.0,82315008.0,dom
155,0,/features/features.6/features.6.,1,2,490.06781,104.1708243475774,2.4269506069439424,131712.0,84658912.0,82204416.0,dom
156,0,/features/features.6/features.6.,1,2,489.4131540000001,103.75541501027448,2.4250521859105145,37632.0,84880096.0,81983232.0,dom
157,0,/features/features.6/features.6.,1,2,490.44280200000003,104.3668473563802,2.423156732539859,150528.0,85101280.0,81762048.0,dom
158,0,/features/features.6/features.6.,1,2,516.751602,108.61060715454701,2.1242895472930794,150528.0,118278880.0,48584448.0,dom
159,0,/features/features.6/features.6.,1,2,516.62117,108.52496249312024,2.124176918617132,131712.0,118389472.0,48473856.0,dom
160,0,/features/features.6/features.6.,1,2,515.966514,108.10955315581731,2.122722483286426,37632.0,118610656.0,48252672.0,dom
161,0,/features/features.6/features.6.,1,2,516.996162,108.72098550192305,2.1212700383122582,150528.0,118831840.0,48031488.0,dom
162,0,/features/features.6/features.6.,1,2,543.304962,112.96474530008985,1.8886579479920262,150528.0,152009440.0,14853888.0,dom
163,0,/features/features.6/features.6.,1,2,543.3463300000001,112.9795328234861,1.8885757672235182,152928.0,152064736.0,14798592.0,dom
164,0,/features/features.6/features.6.,1,2,543.1745300000001,112.87910063866309,1.8885689191489667,131712.0,152120032.0,14743296.0,dom
165,0,/features/features.7/features.7.,1,2,543.243266,112.89137004746588,1.8862707743960172,112896.0,152562400.0,14300928.0,dom
166,0,/features/features.7/features.7.,1,2,549.2307859999999,114.73468522767133,1.8262678014997387,112896.0,164506336.0,2356992.0,dom
167,0,/features/features.7/features.7.,1,2,549.272154,114.74947275106759,1.8261909604789266,115296.0,164561632.0,2301696.0,dom
168,0,/features/features.7/features.7.,1,2,549.253586,114.74097976624456,1.8261845573524034,112896.0,164616928.0,2246400.0,dom
169,0,/features/features.7/features.7.,1,2,548.8821780000001,114.44109239693458,1.8240356460342089,31360.0,164985568.0,1877760.0,dom
170,0,/Flatten,1,2,548.9726260000001,114.38605124961957,1.8216538904971054,2560.0,165395168.0,1282000.0,dom


==> figures/eval_efficientnet_result_acc.tex <==
3.293103464173603,0.7565918,dom
3.2985538216450836,0.76416016,dom
3.354772116368725,0.7553711,dom
3.354772341458659,0.76501465,dom
3.6863646826209586,0.75720215,dom
4.053987437179409,0.7680664,opt
4.053990724144903,0.7680664,dom
4.195253473439136,0.76660156,nondom
4.809190092952987,0.7541504,nondom
4.809199344294522,0.76013184,nondom
3.9541192472211035,0.7573242,dom
2.829317729834674,0.76220703,dom
2.8293087642196104,0.75756836,dom
1.8261845573524034,0.7618408,dom
3.2627776162884126,0.7557373,edge
1.8216538904971054,0.7624512,sensor


==> figures/eval_googlenet_result.tex <==
0,0,input,1,2,32.622526,9.388133296236745,33.14304804681389,301056.0,150528.0,8214976.0,edge
1,0,/maxpool1/MaxPool,1,2,36.387118,10.102166709403296,36.901785160758934,401408.0,1615040.0,7804160.0,nondom
2,0,/conv2/Relu,1,2,37.139758,10.137591581784145,37.246611303303624,401408.0,1619136.0,7800064.0,nondom
3,0,/maxpool2/MaxPool,1,2,41.59148599999999,10.449654332642186,49.814887876650374,301056.0,1729728.0,7237888.0,nondom
4,0,/inception3a/branch3/branch3.0/c,1,2,41.874126,10.598100794910316,49.931892898087014,326144.0,1732800.0,7234816.0,nondom
5,0,/inception3a/branch3/branch3.1/c,1,2,42.195966,10.72660575642195,50.10843465258821,351232.0,1737408.0,7230208.0,nondom
6,0,/inception3a/branch2/branch2.0/c,1,2,46.090766,12.997300029701139,50.296143694070686,802816.0,1755840.0,7211776.0,nondom
7,0,/maxpool3/MaxPool,1,2,51.484078000000004,11.98143636591673,26.706662564523295,188160.0,2223808.0,6348672.0,nondom
8,0,/inception4c/branch2/branch2.0/c,1,2,53.659274,12.15411574290049,22.779292347615645,134848.0,3187136.0,5385344.0,nondom
9,0,/maxpool4/MaxPool,1,2,56.90973800000002,12.451020999384353,18.510182080959087,81536.0,4869568.0,3454384.0,nondom
10,0,output,1,2,57.778957999999996,12.467832694381283,17.307457991337962,0.0,8214976.0,0.0,sensor
11,0,/conv3/conv/Conv,1,2,48.94204599999999,14.859990332642186,49.814887876650374,1204224.0,1729728.0,7237888.0,dom
12,0,/inception3a/branch3/branch3.0/R,1,2,41.874126,10.598100794910316,49.931892898087014,326144.0,1732800.0,7234816.0,dom
13,0,/inception3a/branch1/Relu,1,2,46.116558,11.606423717975442,39.7602931446893,401408.0,1884864.0,7082752.0,dom
14,0,/inception3b/branch1/Relu,1,2,56.078126000000005,14.737865165916729,26.706662564523295,752640.0,2223808.0,6461568.0,dom
15,0,/inception3b/Concat,1,2,56.078126000000005,14.737865165916729,26.706662564523295,752640.0,2223808.0,6348672.0,dom
16,0,/inception4a/branch3/branch3.0/R,1,2,52.746454,12.634982132804804,26.113042315662813,307328.0,2369728.0,6202752.0,dom
17,0,/inception4a/branch2/branch2.0/R,1,2,52.862538,12.69886362310985,26.08557738860415,319872.0,2376640.0,6195840.0,dom
18,0,/inception4a/branch1/Relu,1,2,53.730298000000005,13.219519623109848,26.08557738860415,426496.0,2376640.0,6195840.0,dom
19,0,/inception4a/branch3/branch3.1/R,1,2,53.730298000000005,13.219519623109848,26.08557738860415,426496.0,2376640.0,6195840.0,dom
20,0,/inception4a/branch4/branch4.1/R,1,2,52.155754,12.18487576293358,25.276218515942215,200704.0,2587072.0,5985408.0,dom
21,0,/inception4a/Concat,1,2,52.155754,12.18487576293358,25.276218515942215,200704.0,2587072.0,5985408.0,dom
22,0,/inception4b/branch2/branch2.0/R,1,2,52.795466,12.430212508655368,24.959665181067397,244608.0,2644416.0,5928064.0,dom
23,0,/inception4b/branch4/branch4.0/M,1,2,54.530122,13.468925580853888,24.91508937540861,454720.0,2656704.0,5915776.0,dom
24,0,/inception4b/branch3/branch3.0/R,1,2,54.530122,13.468925580853888,24.91508937540861,454720.0,2656704.0,5915776.0,dom
25,0,/inception4b/branch3/branch3.1/R,1,2,56.210122000000005,14.258915124126975,24.07661371095736,602112.0,2896320.0,5676160.0,dom
26,0,/inception4b/branch4/branch4.1/R,1,2,54.737898,13.300207367439084,23.911546407529265,401408.0,2929088.0,5643392.0,dom
27,0,/inception4c/branch4/branch4.0/M,1,2,54.997738000000005,13.351865026603512,23.588110082879183,401408.0,3011008.0,5561472.0,dom
28,0,/inception4c/branch3/branch3.0/R,1,2,55.098890000000004,13.410475698802033,23.54829472668907,410816.0,3023296.0,5549184.0,dom
29,0,/inception4c/branch3/branch3.1/R,1,2,54.814354,12.564665465080832,21.881608245690195,200704.0,3495872.0,5076608.0,dom
30,0,/inception4c/branch4/branch4.1/R,1,2,54.814354,12.564665465080832,21.881608245690195,200704.0,3495872.0,5076608.0,dom
31,0,/inception4c/Concat,1,2,54.814354,12.564665465080832,21.881608245690195,200704.0,3495872.0,5076608.0,dom
32,0,/inception4d/branch4/branch4.0/M,1,2,58.44577,14.31331696539341,20.6393236906413,526848.0,3959232.0,4613248.0,dom
33,0,/inception4d/branch3/branch3.0/R,1,2,57.17778600000001,13.477153208705516,20.517904744396144,351232.0,3992000.0,4580480.0,dom
34,0,/inception4d/branch2/branch2.1/R,1,2,57.73929000000001,13.814055608705516,20.517904744396144,420224.0,3992000.0,4580480.0,dom
35,0,/inception4d/branch4/branch4.1/R,1,2,57.67402600000001,13.759027634133156,20.472740137052707,407680.0,4010432.0,4562048.0,dom
36,0,/inception4d/branch3/branch3.1/R,1,2,57.67402600000001,13.759027634133156,20.472740137052707,407680.0,4010432.0,4562048.0,dom
37,0,/inception4d/branch1/conv/Conv,1,2,56.32276200000001,12.809778779854945,20.264574281823485,206976.0,4067776.0,4504704.0,dom
38,0,/inception4d/branch1/Relu,1,2,56.32276200000001,12.809778779854945,20.264574281823485,206976.0,4067776.0,4504704.0,dom
39,0,/inception4e/branch3/branch3.0/R,1,2,56.45886600000001,12.880015215344656,20.22418100156616,219520.0,4084672.0,4456448.0,dom
40,0,/inception4e/branch4/branch4.0/M,1,2,61.449466000000015,15.772816047137932,19.938748165635165,802816.0,4206016.0,4310016.0,dom
41,0,/inception4e/branch2/branch2.1/c,1,2,61.86297000000001,15.594183297657745,18.924483740083566,740096.0,4666816.0,3849216.0,dom
42,0,/inception4e/Concat,1,2,58.900506000000014,13.645481799384353,18.510182080959087,326144.0,4869568.0,3454384.0,dom
43,0,/inception5a/branch3/branch3.1/c,1,2,57.690658000000006,12.62942544706543,17.94038624933979,81536.0,5846464.0,2477488.0,dom
44,0,/inception5a/branch3/branch3.1/R,1,2,57.690658000000006,12.62942544706543,17.94038624933979,81536.0,5846464.0,2477488.0,dom
45,0,/inception5b/branch2/branch2.0/R,1,2,58.426469999999995,12.970814821563248,17.627283085705262,123872.0,6472128.0,1824384.0,dom
46,0,/inception5b/Concat,1,2,58.595342,12.957663094381283,17.307457991337962,100352.0,7190976.0,1026048.0,dom
47,0,/fc/Gemm,1,2,57.795006,12.477461494381282,17.307457991337962,2000.0,8214976.0,1000.0,dom
48,0,/conv1/conv/Conv,1,2,46.187934,15.982656309403296,36.901785160758934,1605632.0,962752.0,7804160.0,dom
49,0,/inception3a/branch4/branch4.1/c,1,2,44.20558199999999,11.807641047013721,49.66940047046857,551936.0,1761984.0,7205632.0,dom
50,0,/inception3a/branch2/branch2.1/c,1,2,47.436462,12.532849906655239,40.5696629796957,602112.0,1872576.0,7095040.0,dom
51,0,/inception3a/branch4/branch4.1/R,1,2,46.116558,11.606423717975442,39.7602931446893,401408.0,1884864.0,7082752.0,dom
52,0,/inception3b/branch4/branch4.1/c,1,2,47.685950000000005,12.180763391547128,38.23471834777076,501760.0,1901248.0,7066368.0,dom
53,0,/inception3b/branch3/branch3.0/c,1,2,48.47054200000001,12.473800598879532,37.51500600240096,551936.0,1909440.0,7058176.0,dom
54,0,/inception3b/branch2/branch2.0/c,1,2,51.609326,13.566405408374262,34.88813468494619,752640.0,1942208.0,7025408.0,dom
55,0,/inception3b/branch1/conv/Conv,1,2,51.48110200000001,12.698805417868993,32.6050665665039,551936.0,1974976.0,6992640.0,dom
56,0,/inception3b/branch4/branch4.1/R,1,2,55.15659000000001,14.904098217868992,32.6050665665039,1003520.0,1974976.0,6942464.0,dom
57,0,/inception3b/branch3/branch3.1/c,1,2,55.07739,14.787642649282013,31.824106888264286,953344.0,2002624.0,6914816.0,dom
58,0,/inception4a/branch3/branch3.0/c,1,2,51.55048600000001,12.01993662411574,26.674747336793224,194432.0,2231488.0,6340992.0,dom
59,0,/inception4a/branch1/conv/Conv,1,2,52.347798,12.431128795616981,26.297630267941294,269696.0,2323648.0,6248832.0,dom
60,0,/inception4a/branch2/branch2.0/c,1,2,52.746454,12.634982132804804,26.113042315662813,307328.0,2369728.0,6202752.0,dom
61,0,/inception4a/branch3/branch3.1/c,1,2,52.862538,12.69886362310985,26.08557738860415,319872.0,2376640.0,6195840.0,dom
62,0,/inception4a/branch2/branch2.1/c,1,2,53.625642,13.087209145253219,25.39122804166599,388864.0,2556352.0,6016128.0,dom
63,0,/inception4a/branch4/branch4.1/c,1,2,52.155754,12.18487576293358,25.276218515942215,200704.0,2587072.0,5985408.0,dom
64,0,/inception4b/branch2/branch2.0/c,1,2,52.795466,12.430212508655368,24.959665181067397,244608.0,2644416.0,5928064.0,dom
65,0,/inception4b/branch3/branch3.0/c,1,2,52.896618,12.488823180853888,24.91508937540861,254016.0,2656704.0,5915776.0,dom
66,0,/inception4b/branch3/branch3.1/c,1,2,54.685362,13.549999405994217,24.865131526599722,470400.0,2670528.0,5901952.0,dom
67,0,/inception4b/branch2/branch2.1/c,1,2,55.495386,13.830073524126975,24.07661371095736,514304.0,2896320.0,5676160.0,dom
68,0,/inception4b/branch4/branch4.1/c,1,2,54.737898,13.300207367439084,23.911546407529265,401408.0,2929088.0,5643392.0,dom
69,0,/inception4b/branch1/conv/Conv,1,2,53.364234,12.371762626603513,23.588110082879183,200704.0,3011008.0,5561472.0,dom
70,0,/inception4c/branch3/branch3.0/c,1,2,55.098890000000004,13.410475698802033,23.54829472668907,410816.0,3023296.0,5549184.0,dom
71,0,/inception4c/branch4/branch4.1/c,1,2,53.830906000000006,12.57431194211414,23.390368407658563,235200.0,3056064.0,5516416.0,dom
72,0,/inception4c/branch1/conv/Conv,1,2,54.561946000000006,12.854327442507314,23.080786445485025,285376.0,3121600.0,5450880.0,dom
73,0,/inception4c/branch2/branch2.1/c,1,2,54.659114,12.4835916399405,21.920287313589874,185024.0,3482048.0,5090432.0,dom
74,0,/inception4c/branch2/branch2.1/R,1,2,54.814354,12.564665465080832,21.881608245690195,200704.0,3495872.0,5076608.0,dom
75,0,/inception4d/branch2/branch2.0/R,1,2,55.421682,12.876658276543473,21.67760374034046,257152.0,3569600.0,5002880.0,dom
76,0,/inception4d/branch2/branch2.1/c,1,2,56.62961000000001,13.257732207284237,20.700573654297106,313600.0,3942848.0,4629632.0,dom
77,0,/inception4d/branch3/branch3.0/c,1,2,56.812266,13.33321456539341,20.6393236906413,326144.0,3959232.0,4613248.0,dom
78,0,/inception4d/branch4/branch4.1/c,1,2,57.17778600000001,13.477153208705516,20.517904744396144,351232.0,3992000.0,4580480.0,dom
79,0,/inception4d/branch3/branch3.1/c,1,2,57.67402600000001,13.759027634133156,20.472740137052707,407680.0,4010432.0,4562048.0,dom
80,0,/inception4d/Concat,1,2,56.32276200000001,12.809778779854945,20.264574281823485,206976.0,4067776.0,4473344.0,dom
81,0,/inception4e/branch3/branch3.0/c,1,2,56.45886600000001,12.880015215344656,20.22418100156616,219520.0,4084672.0,4456448.0,dom
82,0,/inception4e/branch3/branch3.1/c,1,2,56.839042000000006,13.075792906699139,20.136606740125004,257152.0,4121536.0,4419584.0,dom
83,0,/inception4e/branch2/branch2.0/R,1,2,57.51893800000001,13.41449924713793,19.938748165635165,319872.0,4206016.0,4335104.0,dom
84,0,/inception4e/branch3/branch3.1/R,1,2,59.76495400000001,14.762108847137931,19.938748165635165,595840.0,4206016.0,4310016.0,dom
85,0,/inception4e/branch2/branch2.1/R,1,2,61.86297000000001,15.594183297657745,18.924483740083566,740096.0,4666816.0,3786496.0,dom
86,0,/inception4e/branch4/branch4.1/c,1,2,60.31397800000002,14.611857663392026,18.784337769442534,533120.0,4734400.0,3718912.0,dom
87,0,/inception5a/branch2/branch2.0/R,1,2,57.14281800000001,12.559901995455153,18.43070644160562,97216.0,5002688.0,3321264.0,dom
88,0,/inception5a/branch2/branch2.1/c,1,2,57.50154600000002,12.698936551529625,18.205226793433297,112896.0,5463488.0,2860464.0,dom
89,0,/inception5a/branch4/branch4.1/c,1,2,57.73460200000002,12.78134273897329,18.128342866424564,125440.0,5569984.0,2753968.0,dom
90,0,/inception5a/branch1/conv/Conv,1,2,58.200922000000006,12.954519029300538,17.976506862711258,150528.0,5782976.0,2540976.0,dom
91,0,/inception5a/branch3/branch3.0/R,1,2,57.69768200000001,12.639658776410634,17.957706010803353,84672.0,5809600.0,2514352.0,dom
92,0,/inception5a/Concat,1,2,57.690658000000006,12.62942544706543,17.94038624933979,81536.0,5846464.0,2468864.0,dom
93,0,/inception5b/branch3/branch3.0/c,1,2,58.412454,13.060178630270334,17.92166083615301,167776.0,5886400.0,2428928.0,dom
94,0,/inception5b/branch1/conv/Conv,1,2,58.87887,13.317908009357646,17.773253102499062,205408.0,6205888.0,2109440.0,dom
95,0,/inception5b/branch4/branch4.1/c,1,2,58.448406,13.002202196801312,17.699967148860974,136416.0,6312384.0,2002944.0,dom
96,0,/inception5b/branch1/Relu,1,2,58.856885999999996,13.24729019680131,17.699967148860974,186592.0,6312384.0,1984128.0,dom
97,0,/inception5b/branch4/branch4.1/R,1,2,58.426469999999995,12.970814821563248,17.627283085705262,123872.0,6472128.0,1818112.0,dom
98,0,/inception5b/branch2/branch2.1/R,1,2,58.606086,12.97338841818139,17.33164731068295,105056.0,7135680.0,1135744.0,dom
99,0,/Flatten,1,2,57.79539,12.477691894381282,17.307457991337962,2048.0,7190976.0,1026000.0,dom


==> figures/eval_regnet_x_400mf_result.tex <==
0,0,input,1,2,40.976928,11.729227427983234,26.000735820823728,309174.0,154587.0,24804960.0,edge
1,0,/trunk_output/block1/block1-0/ac,1,2,42.10228,11.533871308622432,27.099588004963557,207936.0,1260768.0,23960064.0,nondom
2,0,/trunk_output/block2/block2-0/Ad,1,2,42.98788,11.27492954064769,27.728075202976445,107648.0,1305824.0,23822080.0,nondom
3,0,/trunk_output/block2/block2-1/ac,1,2,44.40076,11.473018071969168,28.309004103390144,107648.0,1350880.0,23723200.0,nondom
4,0,/trunk_output/block3/block3-0/Ad,1,2,45.902623999999996,11.832404903019293,29.423663981757336,72000.0,1627360.0,23393600.0,nondom
5,0,/trunk_output/block3/block3-1/f/,1,2,47.250091999999995,12.589932351072676,29.521384552935537,216000.0,1652960.0,23368000.0,nondom
6,0,/trunk_output/block3/block3-1/Ad,1,2,47.401123999999996,12.419632827496695,30.535516622771866,72000.0,1908960.0,23112000.0,nondom
7,0,/trunk_output/block3/block3-2/f/,1,2,48.74859199999999,13.177160275550076,30.640775211612862,216000.0,1934560.0,23086400.0,nondom
8,0,/trunk_output/block3/block3-2/Ad,1,2,48.899623999999996,13.006860751974095,31.73469792534413,72000.0,2190560.0,22830400.0,nondom
9,0,/trunk_output/block3/block3-3/f/,1,2,50.247091999999995,13.764388200027478,31.84840160834429,216000.0,2216160.0,22804800.0,nondom
10,0,/trunk_output/block3/block3-3/Ad,1,2,50.398123999999996,13.594088676451495,33.03191708988811,72000.0,2472160.0,22548800.0,nondom
11,0,/trunk_output/block3/block3-4/f/,1,2,51.745591999999995,14.35161612450488,33.155124538936555,216000.0,2497760.0,22523200.0,nondom
12,0,/trunk_output/block3/block3-4/Ad,1,2,51.896624,14.181316600928898,34.43970898445909,72000.0,2753760.0,22267200.0,nondom
13,0,/trunk_output/block3/block3-5/f/,1,2,53.244091999999995,14.93884404898228,34.57366351181988,216000.0,2779360.0,22241600.0,nondom
14,0,/trunk_output/block3/block3-5/Ad,1,2,53.395123999999996,14.768544525406298,35.97284050541842,72000.0,3035360.0,21985600.0,nondom
15,0,/trunk_output/block3/block3-6/f/,1,2,54.742592,15.526071973459683,36.11901214501784,216000.0,3060960.0,21960000.0,nondom
16,0,/trunk_output/block3/block3-6/f/,1,2,55.304108,15.653016201830317,36.41878101969672,144000.0,3291360.0,21729600.0,nondom
17,0,/trunk_output/block3/block3-6/ac,1,2,54.893624,15.3557724498837,36.04076354520016,72000.0,3316960.0,21668000.0,nondom
18,0,/trunk_output/block4/block4-0/Ad,1,2,58.779270000000004,15.73034401487632,29.27198238060836,51200.0,5044960.0,19836800.0,nondom
19,0,output,1,2,101.04275799999999,18.959783852582444,9.89683930581194,0.0,24804960.0,0.0,sensor
20,0,/trunk_output/block1/block1-0/f/,1,2,52.583876000000004,18.45326876854584,26.58463711039882,1663488.0,1249504.0,24075296.0,dom
21,0,/trunk_output/block1/block1-0/pr,1,2,43.79468,12.549311308622432,27.099588004963557,415872.0,1260768.0,24064032.0,dom
22,0,/trunk_output/block1/block1-0/Ad,1,2,42.10228,11.533871308622432,27.099588004963557,207936.0,1260768.0,24064032.0,dom
23,0,/trunk_output/block2/block2-0/f/,1,2,45.876751999999996,13.587173475669525,27.195366344700727,623808.0,1262816.0,23865088.0,dom
24,0,/trunk_output/block2/block2-0/f/,1,2,44.377520000000004,12.273403934257278,27.650699770084433,315584.0,1299680.0,23828224.0,dom
25,0,/trunk_output/block2/block2-0/pr,1,2,43.86404,11.80062554064769,27.728075202976445,215296.0,1305824.0,23822080.0,dom
26,0,/trunk_output/block2/block2-0/ac,1,2,43.86404,11.80062554064769,27.728075202976445,215296.0,1305824.0,23822080.0,dom
27,0,/trunk_output/block2/block2-1/f/,1,2,44.942040000000006,12.335610722035591,27.77989985346103,322944.0,1309920.0,23817984.0,dom
28,0,/trunk_output/block2/block2-1/f/,1,2,45.95124,12.515120890581265,28.255188429613362,322944.0,1346784.0,23781120.0,dom
29,0,/trunk_output/block2/block2-1/f/,1,2,45.276920000000004,11.998714071969168,28.309004103390144,215296.0,1350880.0,23777024.0,dom
30,0,/trunk_output/block2/block2-1/Ad,1,2,44.40076,11.473018071969168,28.309004103390144,107648.0,1350880.0,23777024.0,dom
31,0,/trunk_output/block3/block3-0/f/,1,2,46.50428399999999,12.301731398960158,29.287937030935392,179648.0,1591520.0,23429440.0,dom
32,0,/trunk_output/block3/block3-0/pr,1,2,46.48860799999999,12.183995303019293,29.423663981757336,144000.0,1627360.0,23393600.0,dom
33,0,/trunk_output/block3/block3-0/ac,1,2,46.48860799999999,12.183995303019293,29.423663981757336,144000.0,1627360.0,23393600.0,dom
34,0,/trunk_output/block3/block3-1/f/,1,2,47.250091999999995,12.589932351072676,29.521384552935537,216000.0,1652960.0,23368000.0,dom
35,0,/trunk_output/block3/block3-1/f/,1,2,48.397591999999996,13.068466979443311,30.430978736353616,216000.0,1883360.0,23137600.0,dom
36,0,/trunk_output/block3/block3-1/f/,1,2,47.987108,12.771223227496694,30.535516622771866,144000.0,1908960.0,23112000.0,dom
37,0,/trunk_output/block3/block3-1/ac,1,2,47.987108,12.771223227496694,30.535516622771866,144000.0,1908960.0,23112000.0,dom
38,0,/trunk_output/block3/block3-2/f/,1,2,48.74859199999999,13.177160275550076,30.640775211612862,216000.0,1934560.0,23086400.0,dom
39,0,/trunk_output/block3/block3-2/f/,1,2,49.896091999999996,13.655694903920715,31.62180323332939,216000.0,2164960.0,22856000.0,dom
40,0,/trunk_output/block3/block3-2/f/,1,2,49.485608,13.358451151974094,31.73469792534413,144000.0,2190560.0,22830400.0,dom
41,0,/trunk_output/block3/block3-2/ac,1,2,49.485608,13.358451151974094,31.73469792534413,144000.0,2190560.0,22830400.0,dom
42,0,/trunk_output/block3/block3-3/f/,1,2,50.247091999999995,13.764388200027478,31.84840160834429,216000.0,2216160.0,22804800.0,dom
43,0,/trunk_output/block3/block3-3/f/,1,2,51.39459199999999,14.242922828398115,32.90962195071785,216000.0,2446560.0,22574400.0,dom
44,0,/trunk_output/block3/block3-3/f/,1,2,50.98410799999999,13.945679076451496,33.03191708988811,144000.0,2472160.0,22548800.0,dom
45,0,/trunk_output/block3/block3-3/ac,1,2,50.98410799999999,13.945679076451496,33.03191708988811,144000.0,2472160.0,22548800.0,dom
46,0,/trunk_output/block3/block3-4/f/,1,2,51.745591999999995,14.35161612450488,33.155124538936555,216000.0,2497760.0,22523200.0,dom
47,0,/trunk_output/block3/block3-4/f/,1,2,52.893091999999996,14.830150752875515,34.30678845576569,216000.0,2728160.0,22292800.0,dom
48,0,/trunk_output/block3/block3-4/f/,1,2,52.482608,14.532907000928898,34.43970898445909,144000.0,2753760.0,22267200.0,dom
49,0,/trunk_output/block3/block3-4/ac,1,2,52.482608,14.532907000928898,34.43970898445909,144000.0,2753760.0,22267200.0,dom
50,0,/trunk_output/block3/block3-5/f/,1,2,53.244091999999995,14.93884404898228,34.57366351181988,216000.0,2779360.0,22241600.0,dom
51,0,/trunk_output/block3/block3-5/f/,1,2,54.391591999999996,15.417378677352916,35.82784719423173,216000.0,3009760.0,22011200.0,dom
52,0,/trunk_output/block3/block3-5/f/,1,2,53.981108,15.1201349254063,35.97284050541842,144000.0,3035360.0,21985600.0,dom
53,0,/trunk_output/block3/block3-5/ac,1,2,53.981108,15.1201349254063,35.97284050541842,144000.0,3035360.0,21985600.0,dom
54,0,/trunk_output/block3/block3-6/f/,1,2,54.742592,15.526071973459683,36.11901214501784,216000.0,3060960.0,21960000.0,dom
55,0,/trunk_output/block3/block3-6/f/,1,2,55.479608,15.707362849883701,36.04076354520016,144000.0,3316960.0,21704000.0,dom
56,0,/trunk_output/block3/block3-6/Ad,1,2,54.893624,15.3557724498837,36.04076354520016,72000.0,3316960.0,21704000.0,dom
57,0,/trunk_output/block4/block4-0/f/,1,2,56.797334,16.385917443568854,35.12918406146763,252000.0,3380960.0,21539600.0,dom
58,0,/trunk_output/block4/block4-0/f/,1,2,59.195942,15.980347214876321,29.27198238060836,102400.0,5044960.0,19836800.0,dom
59,0,/trunk_output/block4/block4-0/ac,1,2,59.195942,15.980347214876321,29.27198238060836,102400.0,5044960.0,19836800.0,dom
60,0,/trunk_output/block4/block4-1/f/,1,2,63.075942,16.296651491031422,24.849437259643814,102400.0,6804960.0,18076800.0,dom
61,0,/trunk_output/block4/block4-1/ac,1,2,63.075942,16.296651491031422,24.849437259643814,102400.0,6804960.0,18076800.0,dom
62,0,/trunk_output/block4/block4-2/f/,1,2,63.932614,16.588403678484788,24.460427431293102,153600.0,6964960.0,17916800.0,dom
63,0,/trunk_output/block4/block4-2/f/,1,2,66.932614,16.82120997973316,21.890287629623337,153600.0,8404960.0,16476800.0,dom
64,0,/trunk_output/block4/block4-2/f/,1,2,66.955942,16.612955767186524,21.587846560494757,102400.0,8564960.0,16316800.0,dom
65,0,/trunk_output/block4/block4-2/ac,1,2,66.955942,16.612955767186524,21.587846560494757,102400.0,8564960.0,16316800.0,dom
66,0,/trunk_output/block4/block4-3/f/,1,2,70.835942,16.929260043341625,19.083109997336,102400.0,10324960.0,14556800.0,dom
67,0,/trunk_output/block4/block4-3/ac,1,2,70.835942,16.929260043341625,19.083109997336,102400.0,10324960.0,14556800.0,dom
68,0,/trunk_output/block4/block4-4/f/,1,2,71.69261399999999,17.22101223079499,18.852856471695453,153600.0,10484960.0,14396800.0,dom
69,0,/trunk_output/block4/block4-4/f/,1,2,74.69261399999999,17.45381853204336,17.288367902001234,153600.0,11924960.0,12956800.0,dom
70,0,/trunk_output/block4/block4-4/f/,1,2,74.715942,17.245564319496726,17.09917315238304,102400.0,12084960.0,12796800.0,dom
71,0,/trunk_output/block4/block4-4/ac,1,2,74.715942,17.245564319496726,17.09917315238304,102400.0,12084960.0,12796800.0,dom
72,0,/trunk_output/block4/block4-5/f/,1,2,78.59594200000001,17.561868595651827,15.488900963347685,102400.0,13844960.0,11036800.0,dom
73,0,/trunk_output/block4/block4-5/ac,1,2,78.59594200000001,17.561868595651827,15.488900963347685,102400.0,13844960.0,11036800.0,dom
74,0,/trunk_output/block4/block4-6/f/,1,2,82.452614,18.086427084353563,14.285232669298578,153600.0,15444960.0,9436800.0,dom
75,0,/trunk_output/block4/block4-6/f/,1,2,82.475942,17.878172871806928,14.15581246153158,102400.0,15604960.0,9276800.0,dom
76,0,/trunk_output/block4/block4-6/ac,1,2,82.475942,17.878172871806928,14.15581246153158,102400.0,15604960.0,9276800.0,dom
77,0,/trunk_output/block4/block4-7/f/,1,2,86.33261399999999,18.402731360508664,13.143651169600943,153600.0,17204960.0,7676800.0,dom
78,0,/trunk_output/block4/block4-7/f/,1,2,86.355942,18.19447714796203,13.034009902719365,102400.0,17364960.0,7516800.0,dom
79,0,/trunk_output/block4/block4-7/ac,1,2,86.355942,18.19447714796203,13.034009902719365,102400.0,17364960.0,7516800.0,dom
80,0,/trunk_output/block4/block4-8/f/,1,2,90.21261399999999,18.71903563666377,12.171023325035943,153600.0,18964960.0,5916800.0,dom
81,0,/trunk_output/block4/block4-8/f/,1,2,90.235942,18.51078142411713,12.076950463730745,102400.0,19124960.0,5756800.0,dom
82,0,/trunk_output/block4/block4-8/ac,1,2,90.235942,18.51078142411713,12.076950463730745,102400.0,19124960.0,5756800.0,dom
83,0,/trunk_output/block4/block4-9/ac,1,2,94.115942,18.827085700272235,11.250826373197112,102400.0,20884960.0,3996800.0,dom
84,0,/trunk_output/block4/block4-10/f,1,2,97.995942,19.143389976427336,10.530488079698104,102400.0,22644960.0,2236800.0,dom
85,0,/trunk_output/block4/block4-11/f,1,2,101.875942,19.45969425258244,9.89683930581194,102400.0,24404960.0,451200.0,dom
86,0,/trunk_output/block4/block4-11/A,1,2,101.45926999999999,19.209691052582443,9.89683930581194,51200.0,24404960.0,426000.0,dom
87,0,/trunk_output/block4/block4-11/a,1,2,101.45926999999999,19.209691052582443,9.89683930581194,51200.0,24404960.0,402000.0,dom
88,0,/Flatten,1,2,101.04899799999998,18.96352785258244,9.89683930581194,800.0,24404960.0,402000.0,dom
89,0,/stem/stem.0/Conv,1,2,45.034932,14.324951563682946,26.402201098701195,831744.0,571323.0,24804096.0,dom
90,0,/stem/stem.2/Relu,1,2,45.034932,14.324951563682946,26.402201098701195,831744.0,832608.0,24388224.0,dom
91,0,/trunk_output/block1/block1-0/f/,1,2,52.583876000000004,18.45326876854584,26.58463711039882,1663488.0,833632.0,24075296.0,dom
92,0,/trunk_output/block1/block1-0/f/,1,2,48.481792,15.559969861635619,27.004481933866565,1039680.0,1258720.0,24066080.0,dom
93,0,/trunk_output/block1/block1-0/f/,1,2,48.676732,15.576041295057504,27.051951378986747,1039680.0,1259744.0,24065056.0,dom
94,0,/trunk_output/block2/block2-0/f/,1,2,45.876751999999996,13.587173475669525,27.195366344700727,623808.0,1262816.0,23865088.0,dom
95,0,/trunk_output/block2/block2-0/f/,1,2,44.377520000000004,12.273403934257278,27.650699770084433,315584.0,1299680.0,23828224.0,dom
96,0,/trunk_output/block2/block2-0/f/,1,2,44.579359999999994,12.28269311564518,27.702235321070294,315584.0,1303776.0,23824128.0,dom
97,0,/trunk_output/block2/block2-1/f/,1,2,44.942040000000006,12.335610722035591,27.77989985346103,322944.0,1309920.0,23817984.0,dom
98,0,/trunk_output/block2/block2-1/f/,1,2,45.07508,11.989424890581265,28.255188429613362,215296.0,1346784.0,23781120.0,dom
99,0,/trunk_output/block3/block3-0/f/,1,2,46.96119999999999,12.791176190859922,28.44444444444445,376768.0,1361120.0,23659840.0,dom
100,0,/trunk_output/block3/block3-0/f/,1,2,46.50428399999999,12.301731398960158,29.287937030935392,179648.0,1591520.0,23429440.0,dom
101,0,/trunk_output/block3/block3-0/f/,1,2,46.679784,12.35607804701354,29.384756657483937,179648.0,1617120.0,23403840.0,dom
102,0,/trunk_output/block3/block3-1/f/,1,2,47.81160799999999,12.716876579443312,30.430978736353616,144000.0,1883360.0,23137600.0,dom
103,0,/trunk_output/block3/block3-2/f/,1,2,49.31010799999999,13.304104503920714,31.62180323332939,144000.0,2164960.0,22856000.0,dom
104,0,/trunk_output/block3/block3-3/f/,1,2,50.80860799999999,13.891332428398114,32.90962195071785,144000.0,2446560.0,22574400.0,dom
105,0,/trunk_output/block3/block3-4/f/,1,2,52.307108,14.478560352875515,34.30678845576569,144000.0,2728160.0,22292800.0,dom
106,0,/trunk_output/block3/block3-5/f/,1,2,53.80560799999999,15.065788277352915,35.82784719423173,144000.0,3009760.0,22011200.0,dom
107,0,/trunk_output/block4/block4-0/f/,1,2,56.797334,16.385917443568854,35.12918406146763,252000.0,3380960.0,21500800.0,dom
108,0,/trunk_output/block4/block4-0/f/,1,2,58.74925399999999,16.023172092221664,30.06039735035633,123200.0,4820960.0,20060800.0,dom
109,0,/trunk_output/block4/block4-0/pr,1,2,58.755942000000005,15.938598227422954,29.830835299185374,102400.0,4884960.0,19996800.0,dom
110,0,/trunk_output/block4/block4-1/f/,1,2,60.052614,16.272099402329687,28.73368357778035,153600.0,5204960.0,19676800.0,dom
111,0,/trunk_output/block4/block4-1/f/,1,2,62.635942,16.254902503578055,25.25102039373411,102400.0,6644960.0,18236800.0,dom
112,0,/trunk_output/block4/block4-1/Ad,1,2,62.65927000000001,16.046648291031424,24.849437259643814,51200.0,6804960.0,18076800.0,dom
113,0,/trunk_output/block4/block4-2/f/,1,2,63.932614,16.588403678484788,24.460427431293102,153600.0,6964960.0,17916800.0,dom
114,0,/trunk_output/block4/block4-2/f/,1,2,66.515942,16.571206779733156,21.890287629623337,102400.0,8404960.0,16476800.0,dom
115,0,/trunk_output/block4/block4-2/Ad,1,2,66.53927,16.36295256718652,21.587846560494757,51200.0,8564960.0,16316800.0,dom
116,0,/trunk_output/block4/block4-3/f/,1,2,67.812614,16.90470795463989,21.293648785963907,153600.0,8724960.0,16156800.0,dom
117,0,/trunk_output/block4/block4-3/f/,1,2,70.39594199999999,16.887511055888258,19.319057322734125,102400.0,10164960.0,14716800.0,dom
118,0,/trunk_output/block4/block4-3/Ad,1,2,70.41927,16.679256843341626,19.083109997336,51200.0,10324960.0,14556800.0,dom
119,0,/trunk_output/block4/block4-4/f/,1,2,71.69261399999999,17.22101223079499,18.852856471695453,153600.0,10484960.0,14396800.0,dom
120,0,/trunk_output/block4/block4-4/f/,1,2,74.275942,17.20381533204336,17.288367902001234,102400.0,11924960.0,12956800.0,dom
121,0,/trunk_output/block4/block4-4/Ad,1,2,74.29927,16.995561119496724,17.09917315238304,51200.0,12084960.0,12796800.0,dom
122,0,/trunk_output/block4/block4-5/f/,1,2,75.572614,17.53731650695009,16.914074471993338,153600.0,12244960.0,12636800.0,dom
123,0,/trunk_output/block4/block4-5/f/,1,2,78.15594200000001,17.52011960819846,15.643978100933696,102400.0,13684960.0,11196800.0,dom
124,0,/trunk_output/block4/block4-5/Ad,1,2,78.17927,17.31186539565183,15.488900963347685,51200.0,13844960.0,11036800.0,dom
125,0,/trunk_output/block4/block4-6/f/,1,2,79.452614,17.853620783105193,15.33686817471024,153600.0,14004960.0,10876800.0,dom
126,0,/trunk_output/block4/block4-6/f/,1,2,82.035942,17.83642388435356,14.285232669298578,102400.0,15444960.0,9436800.0,dom
127,0,/trunk_output/block4/block4-6/Ad,1,2,82.05927,17.628169671806926,14.15581246153158,51200.0,15604960.0,9276800.0,dom
128,0,/trunk_output/block4/block4-7/f/,1,2,83.33261399999999,18.169925059260294,14.028716220955648,153600.0,15764960.0,9116800.0,dom
129,0,/trunk_output/block4/block4-7/f/,1,2,85.915942,18.152728160508662,13.143651169600943,102400.0,17204960.0,7676800.0,dom
130,0,/trunk_output/block4/block4-7/Ad,1,2,85.93927,17.94447394796203,13.034009902719365,51200.0,17364960.0,7516800.0,dom
131,0,/trunk_output/block4/block4-8/f/,1,2,87.21261399999999,18.486229335415395,12.926182706939137,153600.0,17524960.0,7356800.0,dom
132,0,/trunk_output/block4/block4-8/f/,1,2,89.795942,18.469032436663767,12.171023325035943,102400.0,18964960.0,5916800.0,dom
133,0,/trunk_output/block4/block4-8/Ad,1,2,89.81926999999999,18.260778224117132,12.076950463730745,51200.0,19124960.0,5756800.0,dom
134,0,/trunk_output/block4/block4-9/f/,1,2,91.092614,18.8025336115705,11.984320673576347,153600.0,19284960.0,5596800.0,dom
135,0,/trunk_output/block4/block4-9/f/,1,2,93.67594199999999,18.785336712818868,11.332425832672653,102400.0,20724960.0,4156800.0,dom
136,0,/trunk_output/block4/block4-9/Ad,1,2,93.69927,18.577082500272237,11.250826373197112,51200.0,20884960.0,3996800.0,dom
137,0,/trunk_output/block4/block4-10/f,1,2,94.972614,19.1188378877256,11.170393631267094,153600.0,21044960.0,3836800.0,dom
138,0,/trunk_output/block4/block4-10/f,1,2,97.555942,19.101640988973973,10.601939985386288,102400.0,22484960.0,2396800.0,dom
139,0,/trunk_output/block4/block4-10/A,1,2,97.57927,18.893386776427338,10.530488079698104,51200.0,22644960.0,2236800.0,dom
140,0,/trunk_output/block4/block4-10/a,1,2,97.995942,19.143389976427336,10.530488079698104,102400.0,22644960.0,2211200.0,dom
141,0,/trunk_output/block4/block4-11/f,1,2,98.85261399999999,19.435142163880705,10.459992828628918,153600.0,22804960.0,2051200.0,dom
142,0,/trunk_output/block4/block4-11/f,1,2,101.435942,19.417945265129074,9.959925244785085,102400.0,24244960.0,611200.0,dom
143,0,/avgpool/GlobalAveragePool,1,2,101.04899799999998,18.96352785258244,9.89683930581194,800.0,24404960.0,402000.0,dom


==> figures/eval_resnet50_result.tex <==
0,0,input,1,2,83.04548599999998,23.635469507690402,12.407686810132617,301056.0,150528.0,27911360.0,edge
1,0,/maxpool/MaxPool,1,2,86.81007799999998,24.34950292085695,12.89957730665082,401408.0,1615040.0,27901952.0,nondom
2,0,/layer1/layer1.0/conv1/Conv,1,2,90.82972599999998,26.3451325932378,12.94145905115293,802816.0,1619136.0,27897856.0,nondom
3,0,/layer1/layer1.0/conv2/Conv,1,2,94.59292599999998,26.792130266553784,13.331001296839808,802816.0,1656000.0,27860992.0,nondom
4,0,/layer1/layer1.0/Add,1,2,107.147854,31.141041119802168,13.697489305000351,1605632.0,2491584.0,27828224.0,nondom
5,0,/layer1/layer1.1/Add,1,2,116.93217399999999,31.995716857284677,14.547333531952928,1605632.0,2561216.0,27758592.0,nondom
6,0,/layer1/layer1.2/relu_2/Relu,1,2,126.71649400000001,32.85039259476717,15.509608512665764,1605632.0,2630848.0,26484736.0,nondom
7,0,/layer2/layer2.0/relu/Relu,1,2,139.271422,37.09306311116511,16.007909187771492,2408448.0,2663616.0,26451968.0,opt
8,0,/layer2/layer2.0/conv2/Conv,1,2,138.134318,34.806807876411234,15.817338840298023,1806336.0,2811072.0,26304512.0,nondom
9,0,/layer4/layer4.0/downsample/down,1,2,200.09385399999996,35.396860531702586,5.304521998913635,250880.0,15901888.0,12310528.0,nondom
10,0,/layer4/layer4.0/Add,1,2,200.97561399999995,35.343694455863066,5.240756144681766,200704.0,16950464.0,11261952.0,nondom
11,0,output,1,2,206.8688779999999,35.825554064983024,4.833989208989211,0.0,27911360.0,0.0,sensor
12,0,/layer1/layer1.0/relu_1/Relu,1,2,94.59292599999998,26.792130266553784,13.331001296839808,802816.0,1656000.0,27860992.0,dom
13,0,/layer1/layer1.1/conv2/Conv,1,2,130.256238,41.58217823066048,14.338019380414035,3612672.0,2544832.0,27774976.0,dom
14,0,/layer1/layer1.2/conv2/Conv,1,2,140.040558,42.436853968142984,15.271913363046368,3612672.0,2614464.0,26902528.0,dom
15,0,/layer1/layer1.2/conv3/Conv,1,2,139.78411,40.69096219476718,15.509608512665764,3211264.0,2630848.0,26886144.0,dom
16,0,/layer1/layer1.2/Add,1,2,126.71649400000001,32.85039259476717,15.509608512665764,1605632.0,2630848.0,26886144.0,dom
17,0,/layer2/layer2.0/relu_1/Relu,1,2,138.134318,34.806807876411234,15.817338840298023,1806336.0,2811072.0,26304512.0,dom
18,0,/layer2/layer2.0/downsample/down,1,2,145.532494,34.480726298536744,13.28656462585034,1605632.0,3007680.0,26107904.0,dom
19,0,/layer2/layer2.0/relu_2/Relu,1,2,145.532494,34.480726298536744,13.28656462585034,1605632.0,3007680.0,26107904.0,dom
20,0,/layer2/layer2.1/relu/Relu,1,2,150.176558,35.75583238827949,12.613827176440198,1806336.0,3073216.0,26042368.0,dom
21,0,/layer2/layer2.1/conv2/Conv,1,2,153.939758,36.3938263292893,11.723439375750303,1806336.0,3220672.0,25894912.0,dom
22,0,/layer2/layer2.1/relu_2/Relu,1,2,155.316814,35.61704150862692,11.196543224031187,1605632.0,3286208.0,25829376.0,dom
23,0,/layer2/layer2.2/conv3/Conv,1,2,165.101134,36.75335671871709,9.67468297998811,1605632.0,3564736.0,25550848.0,dom
24,0,/layer2/layer2.3/conv2/Conv,1,2,173.50839800000003,38.666456749469646,8.818516344590932,1806336.0,3777728.0,24936448.0,dom
25,0,/layer2/layer2.3/conv3/Conv,1,2,174.88545400000004,37.889671928807275,8.51702860631432,1605632.0,3843264.0,24870912.0,dom
26,0,/layer2/layer2.3/Add,1,2,168.35164600000002,33.96938712880727,8.51702860631432,802816.0,3843264.0,24870912.0,dom
27,0,/layer3/layer3.0/relu_1/Relu,1,2,176.372238,35.20303285438078,7.759117273160655,903168.0,4564160.0,23949312.0,dom
28,0,/layer3/layer3.0/downsample/down,1,2,179.426206,35.15597453311361,7.36583572182833,802816.0,5350592.0,23162880.0,dom
29,0,/layer3/layer3.1/relu/Relu,1,2,181.533198,35.76378546494295,7.2434542352766655,903168.0,5612736.0,22900736.0,dom
30,0,/layer3/layer3.1/conv2/Conv,1,2,182.715918,35.92941132709208,7.067321609494862,903168.0,6202560.0,22310912.0,dom
31,0,/layer3/layer3.1/conv3/Conv,1,2,183.189406,35.56645546618031,6.95458268052984,802816.0,6464704.0,22048768.0,dom
32,0,/layer3/layer3.1/relu_2/Relu,1,2,183.189406,35.56645546618031,6.95458268052984,802816.0,6464704.0,22048768.0,dom
33,0,/layer3/layer3.2/relu/Relu,1,2,185.29639799999998,36.17426639800965,6.845384130099538,903168.0,6726848.0,21786624.0,dom
34,0,/layer3/layer3.2/conv2/Conv,1,2,186.47911799999997,36.339892260158784,6.687868100260239,903168.0,7316672.0,21196800.0,dom
35,0,/layer3/layer3.2/conv3/Conv,1,2,186.95260599999997,35.97693639924701,6.586823823013626,802816.0,7578816.0,20934656.0,dom
36,0,/layer3/layer3.2/relu_2/Relu,1,2,186.95260599999997,35.97693639924701,6.586823823013626,802816.0,7578816.0,20934656.0,dom
37,0,/layer3/layer3.3/relu/Relu,1,2,189.05959799999997,36.58474733107635,6.488787375415284,903168.0,7840960.0,20672512.0,dom
38,0,/layer3/layer3.3/conv2/Conv,1,2,190.24231799999995,36.750373193225485,6.34708501234889,903168.0,8430784.0,20082688.0,dom
39,0,/layer3/layer3.3/conv3/Conv,1,2,190.71580599999996,36.38741733231371,6.2560057655349155,802816.0,8692928.0,19820544.0,dom
40,0,/layer3/layer3.3/relu_2/Relu,1,2,190.71580599999996,36.38741733231371,6.2560057655349155,802816.0,8692928.0,19820544.0,dom
41,0,/layer3/layer3.4/relu/Relu,1,2,192.82279799999995,36.99522826414305,6.167503473537958,903168.0,8955072.0,19558400.0,dom
42,0,/layer3/layer3.4/conv2/Conv,1,2,194.00551799999994,37.16085412629219,6.039347557204702,903168.0,9544896.0,18968576.0,dom
43,0,/layer3/layer3.4/conv3/Conv,1,2,194.47900599999994,36.79789826538041,5.956828717823596,802816.0,9807040.0,18706432.0,dom
44,0,/layer3/layer3.5/relu/Relu,1,2,196.58599799999993,37.40570919720976,5.876534480683598,903168.0,10069184.0,18243584.0,dom
45,0,/layer3/layer3.5/conv2/Conv,1,2,197.76871799999992,37.571335059358894,5.7600713695882995,903168.0,10659008.0,17653760.0,dom
46,0,/layer3/layer3.5/conv3/Conv,1,2,198.24220599999992,37.20837919844712,5.684960414483644,802816.0,10921152.0,17391616.0,dom
47,0,/layer3/layer3.5/Add,1,2,194.97519799999995,35.24817439844712,5.684960414483644,401408.0,10921152.0,17391616.0,dom
48,0,/layer4/layer4.0/relu_2/Relu,1,2,202.60911799999997,36.323796855863066,5.240756144681766,401408.0,16950464.0,11261952.0,dom
49,0,/layer4/layer4.1/conv3/Conv,1,2,206.37231799999995,37.05466746042305,5.029161087650635,401408.0,21406912.0,6805504.0,dom
50,0,/layer4/layer4.2/conv2/Conv,1,2,209.25375799999995,37.83870414082254,4.888189508459307,451584.0,24814784.0,3297280.0,dom
51,0,/avgpool/GlobalAveragePool,1,2,206.90190199999992,35.845368464983025,4.833989208989211,4096.0,25863360.0,2051048.0,dom
52,0,/fc/Gemm,1,2,206.88492599999992,35.835182864983025,4.833989208989211,2000.0,27911360.0,1000.0,dom
53,0,/conv1/Conv,1,2,96.61089399999997,30.229992520856953,12.89957730665082,1605632.0,962752.0,27901952.0,dom
54,0,/layer1/layer1.0/conv3/Conv,1,2,107.404302,32.88693289317798,13.511760636457975,2007040.0,1672384.0,27844608.0,dom
55,0,/layer1/layer1.0/downsample/down,1,2,120.21547,38.98161071980217,13.697489305000351,3211264.0,1889472.0,27828224.0,dom
56,0,/layer1/layer1.1/conv1/Conv,1,2,126.49303800000001,41.1351805573445,13.88839507928607,3612672.0,2507968.0,27811840.0,dom
57,0,/layer1/layer1.1/relu_1/Relu,1,2,117.18862200000001,33.74160863066048,14.338019380414035,2007040.0,2544832.0,27774976.0,dom
58,0,/layer1/layer1.1/relu_2/Relu,1,2,129.99979,39.83628645728467,14.547333531952928,3211264.0,2561216.0,26955776.0,dom
59,0,/layer1/layer1.2/conv1/Conv,1,2,136.277358,41.989856294827,14.762849584278156,3612672.0,2577600.0,26939392.0,dom
60,0,/layer1/layer1.2/relu_1/Relu,1,2,126.972942,34.59628436814299,15.271913363046368,2007040.0,2614464.0,26902528.0,dom
61,0,/layer2/layer2.0/conv3/Conv,1,2,146.045182,37.95030785574886,14.873020103563814,2408448.0,2876608.0,26238976.0,dom
62,0,/layer2/layer2.0/Add,1,2,138.99868600000002,30.560441498536747,13.28656462585034,802816.0,3007680.0,26107904.0,dom
63,0,/layer2/layer2.1/conv1/Conv,1,2,150.176558,35.75583238827949,12.613827176440198,1806336.0,3073216.0,26042368.0,dom
64,0,/layer2/layer2.1/relu_1/Relu,1,2,147.40595000000002,32.47354152928929,11.723439375750303,1003520.0,3220672.0,25894912.0,dom
65,0,/layer2/layer2.1/Add,1,2,148.783006,31.696756708626918,11.196543224031187,802816.0,3286208.0,25829376.0,dom
66,0,/layer2/layer2.2/conv1/Conv,1,2,159.960878,36.89214759836966,10.714971472459952,1806336.0,3351744.0,25763840.0,dom
67,0,/layer2/layer2.2/relu_1/Relu,1,2,157.19027000000003,33.60985673937947,10.065579262007834,1003520.0,3499200.0,25616384.0,dom
68,0,/layer2/layer2.2/Add,1,2,158.567326,32.833071918717096,9.67468297998811,802816.0,3564736.0,25550848.0,dom
69,0,/layer2/layer2.2/relu_2/Relu,1,2,165.101134,36.75335671871709,9.67468297998811,1605632.0,3564736.0,25149440.0,dom
70,0,/layer2/layer2.3/conv1/Conv,1,2,169.74519800000002,38.028462808459835,9.313012588212855,1806336.0,3630272.0,25083904.0,dom
71,0,/layer2/layer2.3/relu_1/Relu,1,2,166.97459000000003,34.74617194946965,8.818516344590932,1003520.0,3777728.0,24936448.0,dom
72,0,/layer2/layer2.3/relu_2/Relu,1,2,168.35164600000002,33.96938712880727,8.51702860631432,802816.0,3843264.0,24670208.0,dom
73,0,/layer3/layer3.0/relu/Relu,1,2,177.639566,36.490625292753556,7.971938775510203,1204224.0,3974336.0,24539136.0,dom
74,0,/layer3/layer3.0/conv2/Conv,1,2,176.372238,35.20303285438078,7.759117273160655,903168.0,4564160.0,23949312.0,dom
75,0,/layer3/layer3.0/conv3/Conv,1,2,180.112526,36.800156993469,7.623438719750196,1204224.0,4826304.0,23687168.0,dom
76,0,/layer3/layer3.0/Add,1,2,176.15919800000003,33.19576973311361,7.36583572182833,401408.0,5350592.0,23162880.0,dom
77,0,/layer3/layer3.1/conv1/Conv,1,2,181.533198,35.76378546494295,7.2434542352766655,903168.0,5612736.0,22900736.0,dom
78,0,/layer3/layer3.1/relu_1/Relu,1,2,179.44891,33.96920652709208,7.067321609494862,501760.0,6202560.0,22310912.0,dom
79,0,/layer3/layer3.1/Add,1,2,179.92239800000002,33.60625066618031,6.95458268052984,401408.0,6464704.0,22048768.0,dom
80,0,/layer3/layer3.2/conv1/Conv,1,2,185.29639799999998,36.17426639800965,6.845384130099538,903168.0,6726848.0,21786624.0,dom
81,0,/layer3/layer3.2/relu_1/Relu,1,2,183.21211,34.379687460158785,6.687868100260239,501760.0,7316672.0,21196800.0,dom
82,0,/layer3/layer3.2/Add,1,2,183.685598,34.01673159924701,6.586823823013626,401408.0,7578816.0,20934656.0,dom
83,0,/layer3/layer3.3/conv1/Conv,1,2,189.05959799999997,36.58474733107635,6.488787375415284,903168.0,7840960.0,20672512.0,dom
84,0,/layer3/layer3.3/relu_1/Relu,1,2,186.97530999999998,34.790168393225485,6.34708501234889,501760.0,8430784.0,20082688.0,dom
85,0,/layer3/layer3.3/Add,1,2,187.44879799999998,34.42721253231371,6.2560057655349155,401408.0,8692928.0,19820544.0,dom
86,0,/layer3/layer3.4/conv1/Conv,1,2,192.82279799999995,36.99522826414305,6.167503473537958,903168.0,8955072.0,19558400.0,dom
87,0,/layer3/layer3.4/relu_1/Relu,1,2,190.73850999999996,35.200649326292194,6.039347557204702,501760.0,9544896.0,18968576.0,dom
88,0,/layer3/layer3.4/Add,1,2,191.21199799999997,34.83769346538041,5.956828717823596,401408.0,9807040.0,18706432.0,dom
89,0,/layer3/layer3.4/relu_2/Relu,1,2,194.47900599999994,36.79789826538041,5.956828717823596,802816.0,9807040.0,18505728.0,dom
90,0,/layer3/layer3.5/conv1/Conv,1,2,196.58599799999993,37.40570919720976,5.876534480683598,903168.0,10069184.0,18243584.0,dom
91,0,/layer3/layer3.5/relu_1/Relu,1,2,194.50170999999995,35.611130259358895,5.7600713695882995,501760.0,10659008.0,17653760.0,dom
92,0,/layer3/layer3.5/relu_2/Relu,1,2,194.97519799999995,35.24817439844712,5.684960414483644,401408.0,10921152.0,17291264.0,dom
93,0,/layer4/layer4.0/conv1/Conv,1,2,199.18918199999996,36.4637962621058,5.540465789175084,602112.0,11445440.0,16766976.0,dom
94,0,/layer4/layer4.0/conv2/Conv,1,2,199.14687799999996,36.051074059137136,5.436824963812494,451584.0,13804736.0,14407680.0,dom
95,0,/layer4/layer4.1/conv1/Conv,1,2,204.30783799999995,36.80820950646707,5.178505143705591,451584.0,17999040.0,10213376.0,dom
96,0,/layer4/layer4.1/relu_1/Relu,1,2,203.85705399999995,36.12773113626256,5.087852974887987,250880.0,20358336.0,7854080.0,dom
97,0,/layer4/layer4.1/Add,1,2,204.73881399999993,36.07456506042305,5.029161087650635,200704.0,21406912.0,6805504.0,dom
98,0,/layer4/layer4.1/relu_2/Relu,1,2,206.37231799999995,37.05466746042305,5.029161087650635,401408.0,21406912.0,6705152.0,dom
99,0,/layer4/layer4.2/relu/Relu,1,2,208.07103799999993,37.53908011102705,4.971807860706651,451584.0,22455488.0,5656576.0,dom
100,0,/layer4/layer4.2/relu_1/Relu,1,2,207.62025399999993,36.85860174082254,4.888189508459307,250880.0,24814784.0,3297280.0,dom
101,0,/Flatten,1,2,206.90190199999992,35.845368464983025,4.833989208989211,4096.0,25863360.0,2050000.0,dom


==> figures/eval_resnet50_result_acc.tex <==
0,0,input,1,2,83.04548599999998,23.635469507690402,12.407686810132617,301056.0,150528.0,27911360.0,0.8550,edge
1,0,/maxpool/MaxPool,1,2,86.81007799999998,24.34950292085695,12.89957730665082,401408.0,1615040.0,27901952.0,0.8602,nondom
4,0,/layer1/layer1.0/Add,1,2,107.147854,31.141041119802168,13.697489305000351,1605632.0,2491584.0,27828224.0,0.8660,nondom
5,0,/layer1/layer1.1/Add,1,2,116.93217399999999,31.995716857284677,14.547333531952928,1605632.0,2561216.0,27758592.0,0.8661,nondom
10,0,/layer4/layer4.0/Add,1,2,200.97561399999995,35.343694455863066,5.240756144681766,200704.0,16950464.0,11261952.0,0.8729,nondom
11,0,output,1,2,206.8688779999999,35.825554064983024,4.833989208989211,0.0,27911360.0,0.0,0.8734,sensor
16,0,/layer1/layer1.2/Add,1,2,126.71649400000001,32.85039259476717,15.509608512665764,1605632.0,2630848.0,26886144.0,0.8672,opt
26,0,/layer2/layer2.3/Add,1,2,168.35164600000002,33.96938712880727,8.51702860631432,802816.0,3843264.0,24870912.0,0.8691,dom
47,0,/layer3/layer3.5/Add,1,2,194.97519799999995,35.24817439844712,5.684960414483644,401408.0,10921152.0,17391616.0,0.8730,dom
51,0,/avgpool/GlobalAveragePool,1,2,206.90190199999992,35.845368464983025,4.833989208989211,4096.0,25863360.0,2051048.0,0.8734,dom
52,0,/fc/Gemm,1,2,206.88492599999992,35.835182864983025,4.833989208989211,2000.0,27911360.0,1000.0,0.8734,dom
53,0,/conv1/Conv,1,2,96.61089399999997,30.229992520856953,12.89957730665082,1605632.0,962752.0,27901952.0,0.8550,dom
62,0,/layer2/layer2.0/Add,1,2,138.99868600000002,30.560441498536747,13.28656462585034,802816.0,3007680.0,26107904.0,0.8704,nondom
65,0,/layer2/layer2.1/Add,1,2,148.783006,31.696756708626918,11.196543224031187,802816.0,3286208.0,25829376.0,0.8693,dom
68,0,/layer2/layer2.2/Add,1,2,158.567326,32.833071918717096,9.67468297998811,802816.0,3564736.0,25550848.0,0.8704,dom
76,0,/layer3/layer3.0/Add,1,2,176.15919800000003,33.19576973311361,7.36583572182833,401408.0,5350592.0,23162880.0,0.8713,dom
79,0,/layer3/layer3.1/Add,1,2,179.92239800000002,33.60625066618031,6.95458268052984,401408.0,6464704.0,22048768.0,0.8713,dom
82,0,/layer3/layer3.2/Add,1,2,183.685598,34.01673159924701,6.586823823013626,401408.0,7578816.0,20934656.0,0.8719,dom
85,0,/layer3/layer3.3/Add,1,2,187.44879799999998,34.42721253231371,6.2560057655349155,401408.0,8692928.0,19820544.0,0.8732,dom
88,0,/layer3/layer3.4/Add,1,2,191.21199799999997,34.83769346538041,5.956828717823596,401408.0,9807040.0,18706432.0,0.8708,dom
97,0,/layer4/layer4.1/Add,1,2,204.73881399999993,36.07456506042305,5.029161087650635,200704.0,21406912.0,6805504.0,0.8733,dom
101,0,/Flatten,1,2,206.90190199999992,35.845368464983025,4.833989208989211,4096.0,25863360.0,2050000.0,0.8734,dom


==> figures/eval_squeezenet1_1_result.tex <==
0,0,/features/features.3/squeeze/Con,1,2,9.296391999999999,2.7765819353158716,141.25251429475446,100352.0,1637184.0,2031616.0,opt
1,0,/features/features.4/squeeze/Con,1,2,10.801672,2.8896526264994646,158.05578737071033,100352.0,1649472.0,2019328.0,nondom
2,0,/features/features.6/squeeze/Con,1,2,11.71052,2.730213720142194,176.52094862357788,50176.0,1663808.0,1603584.0,nondom
3,0,/features/features.9/squeeze/Con,1,2,14.114152,2.9905334464599855,102.55558256185896,18816.0,1766208.0,1491776.0,nondom
4,0,output,1,2,16.955048000000005,3.4592531977525196,58.98086955495983,0.0,2865984.0,0.0,sensor
5,0,/features/features.1/Relu,1,2,21.593656,10.246915549966898,75.17550096577966,1634432.0,1636160.0,2032640.0,dom
6,0,/features/features.3/squeeze_act,1,2,9.296391999999999,2.7765819353158716,141.25251429475446,100352.0,1637184.0,2031616.0,dom
7,0,/features/features.3/expand3x3_a,1,2,16.142616,6.266123734997681,153.04453014257933,802816.0,1647424.0,2021376.0,dom
8,0,/features/features.3/Concat,1,2,16.142616,6.266123734997681,153.04453014257933,802816.0,1647424.0,2021376.0,dom
9,0,/features/features.4/squeeze_act,1,2,10.801672,2.8896526264994646,158.05578737071033,100352.0,1649472.0,2019328.0,dom
10,0,/features/features.4/Concat,1,2,17.647896,6.379194426181273,153.04453014257933,802816.0,1659712.0,1607680.0,dom
11,0,/features/features.6/squeeze_act,1,2,11.71052,2.730213720142194,176.52094862357788,50176.0,1663808.0,1603584.0,dom
12,0,/features/features.6/expand3x3_a,1,2,15.918327999999999,4.8580008771944865,139.4635951204477,451584.0,1700672.0,1566720.0,dom
13,0,/features/features.6/expand1x1_a,1,2,15.698008,4.623776465757008,134.74891560810164,401408.0,1704768.0,1562624.0,dom
14,0,/features/features.6/Concat,1,2,15.698008,4.623776465757008,134.74891560810164,401408.0,1704768.0,1562624.0,dom
15,0,/features/features.7/squeeze_act,1,2,13.215800000000002,2.9567336730894116,126.2152955268037,50176.0,1712960.0,1554432.0,dom
16,0,/features/features.7/expand3x3_a,1,2,17.203288,4.850296418704225,103.31507067267408,401408.0,1753920.0,1504064.0,dom
17,0,/features/features.7/Concat,1,2,17.203288,4.850296418704225,103.31507067267408,401408.0,1753920.0,1504064.0,dom
18,0,/features/features.9/squeeze_act,1,2,14.114152,2.9905334464599855,102.55558256185896,18816.0,1766208.0,1491776.0,dom
19,0,/features/features.9/expand3x3_a,1,2,15.370952000000003,3.6650067206688286,97.19674857436667,150528.0,1858368.0,1399616.0,dom
20,0,/features/features.9/expand1x1_a,1,2,15.370952000000003,3.6650067206688286,97.19674857436667,150528.0,1858368.0,1399616.0,dom
21,0,/features/features.9/Concat,1,2,15.370952000000003,3.6650067206688286,97.19674857436667,150528.0,1858368.0,1399616.0,dom
22,0,/features/features.10/squeeze_ac,1,2,14.335912,3.0326953589106296,96.19149032361702,18816.0,1876800.0,1381184.0,dom
23,0,/features/features.10/expand3x3_,1,2,15.592712000000002,3.707168633119472,91.46176943768387,150528.0,1968960.0,1289024.0,dom
24,0,/features/features.10/expand1x1_,1,2,15.592712000000002,3.707168633119472,91.46176943768387,150528.0,1968960.0,1289024.0,dom
25,0,/features/features.10/Concat,1,2,15.592712000000002,3.707168633119472,91.46176943768387,150528.0,1968960.0,1289024.0,dom
26,0,/features/features.11/squeeze_ac,1,2,14.621000000000002,3.1088722111845932,90.27804735805806,25088.0,1993536.0,1264448.0,dom
27,0,/features/features.11/expand3x3_,1,2,16.426584000000002,4.020543190249452,82.77864741345698,200704.0,2157376.0,1100608.0,dom
28,0,/features/features.11/expand1x1_,1,2,16.426584000000002,4.020543190249452,82.77864741345698,200704.0,2157376.0,1100608.0,dom
29,0,/features/features.11/Concat,1,2,16.426584000000002,4.020543190249452,82.77864741345698,200704.0,2157376.0,1100608.0,dom
30,0,/features/features.12/squeeze_ac,1,2,15.158600000000003,3.1843794335615594,80.85950418569222,25088.0,2190144.0,1067840.0,dom
31,0,/features/features.12/expand3x3_,1,2,16.964184000000003,4.096050412626418,74.79067958551003,200704.0,2353984.0,904000.0,dom
32,0,/features/features.12/expand1x1_,1,2,16.964184000000003,4.096050412626418,74.79067958551003,200704.0,2353984.0,904000.0,dom
33,0,/features/features.12/Concat,1,2,16.964184000000003,4.096050412626418,74.79067958551003,200704.0,2353984.0,904000.0,dom
34,0,/classifier/classifier.3/GlobalA,1,2,16.971096000000003,3.46888199775252,58.98086955495983,2000.0,2865984.0,2000.0,dom
35,0,input,1,2,10.233322999999999,3.703410938204118,129.5866380625761,309174.0,154587.0,2865984.0,edge
36,0,/features/features.0/Conv,1,2,21.593656,10.246915549966898,75.17550096577966,1634432.0,973531.0,2247744.0,dom
37,0,/features/features.2/MaxPool,1,2,11.558488,4.225814749966899,140.0120970451847,401408.0,1636160.0,2032640.0,dom
38,0,/features/features.3/expand1x1/C,1,2,12.75156,4.757389397988364,142.51510660129975,501760.0,1638208.0,2030592.0,dom
39,0,/features/features.3/expand3x3/C,1,2,16.142616,6.266123734997681,153.04453014257933,802816.0,1647424.0,2021376.0,dom
40,0,/features/features.4/expand1x1/C,1,2,14.25684,4.8704600891719565,159.63832341447215,501760.0,1650496.0,2018304.0,dom
41,0,/features/features.5/MaxPool,1,2,12.747384,3.4388872261812726,175.44844622856021,200704.0,1659712.0,1607680.0,dom
42,0,/features/features.6/expand3x3/C,1,2,14.284824,3.877898477194487,139.4635951204477,250880.0,1700672.0,1566720.0,dom
43,0,/features/features.6/expand1x1/C,1,2,15.698008,4.623776465757008,134.74891560810164,401408.0,1704768.0,1562624.0,dom
44,0,/features/features.7/squeeze/Con,1,2,13.215800000000002,2.9567336730894116,126.2152955268037,50176.0,1712960.0,1554432.0,dom
45,0,/features/features.7/expand1x1/C,1,2,15.037464,3.947699661651933,122.34136912226185,250880.0,1717056.0,1550336.0,dom
46,0,/features/features.8/MaxPool,1,2,14.753032000000001,3.3801428187042255,103.31507067267408,100352.0,1753920.0,1504064.0,dom
47,0,/features/features.9/expand1x1/C,1,2,14.745144000000002,3.363252760094366,101.99325416616944,94080.0,1775424.0,1482560.0,dom
48,0,/features/features.9/expand3x3/C,1,2,15.370952000000003,3.6650067206688286,97.19674857436667,150528.0,1858368.0,1399616.0,dom
49,0,/features/features.10/squeeze/Co,1,2,14.335912,3.0326953589106296,96.19149032361702,18816.0,1876800.0,1381184.0,dom
50,0,/features/features.10/expand1x1/,1,2,14.966904000000003,3.40541467254501,95.69661875136964,94080.0,1886016.0,1371968.0,dom
51,0,/features/features.10/expand3x3/,1,2,15.592712000000002,3.707168633119472,91.46176943768387,150528.0,1968960.0,1289024.0,dom
52,0,/features/features.11/squeeze/Co,1,2,14.621000000000002,3.1088722111845932,90.27804735805806,25088.0,1993536.0,1264448.0,dom
53,0,/features/features.11/expand3x3/,1,2,15.733432000000004,3.642692325670038,83.77279143506978,125440.0,2140992.0,1116992.0,dom
54,0,/features/features.11/expand1x1/,1,2,16.426584000000002,4.020543190249452,82.77864741345698,200704.0,2157376.0,1100608.0,dom
55,0,/features/features.12/squeeze/Co,1,2,15.158600000000003,3.1843794335615594,80.85950418569222,25088.0,2190144.0,1067840.0,dom
56,0,/features/features.12/expand1x1/,1,2,16.055992000000003,3.6847742981409732,79.93292029328985,125440.0,2206528.0,1051456.0,dom
57,0,/features/features.12/expand3x3/,1,2,16.964184000000003,4.096050412626418,74.79067958551003,200704.0,2353984.0,904000.0,dom


==> figures/eval_vgg16_result.tex <==
0,0,input,1,2,302.75364599999995,84.30655697985384,3.32996607164169,301056.0,150528.0,144766656.0,edge
1,0,/features/features.0/Conv,1,2,300.62592,83.11694982273431,3.3551930873359446,6422528.0,3363520.0,144764928.0,opt2
2,0,/features/features.3/Relu,1,2,360.83712,77.07222337636603,3.817978340761592,6422528.0,6461120.0,141516800.0,opt
3,0,/features/features.4/MaxPool,1,2,373.904974,84.91293577636603,3.817978340761592,1605632.0,6461120.0,141516800.0,nondom
4,0,/features/features.5/Conv,1,2,417.07818999999995,94.55121731086837,4.100791551188377,3211264.0,6534848.0,141443072.0,nondom
5,0,/features/features.9/MaxPool,1,2,457.68796599999996,86.3057723931646,4.108036765943127,802816.0,6682304.0,139689984.0,nondom
6,0,/features/features.23/MaxPool,1,2,753.843454,117.53178328335808,1.3790918205953795,200704.0,14055104.0,130912256.0,nondom
7,0,output,1,2,766.4029579999999,118.52051243756249,1.3047973117417564,0.0,144766656.0,0.0,sensor
8,0,/features/features.2/Conv,1,2,360.83712,77.07222337636603,3.817978340761592,6422528.0,6461120.0,142319616.0,dom
9,0,/features/features.6/Relu,1,2,417.07818999999995,94.55121731086837,4.100791551188377,3211264.0,6534848.0,141443072.0,dom
10,0,/features/features.11/Relu,1,2,494.327374,92.29189921630368,3.429423022896474,1605632.0,6977216.0,139395072.0,dom
11,0,/features/features.13/Relu,1,2,554.538574,96.38357606922763,2.5777702988068842,1605632.0,7567040.0,138805248.0,dom
12,0,/features/features.15/Relu,1,2,614.749774,100.47525292215157,2.064963418760044,1605632.0,8156864.0,137412608.0,dom
13,0,/features/features.18/Relu,1,2,638.321566,101.34879517925148,1.878149280713901,802816.0,9336512.0,136232960.0,dom
14,0,/features/features.20/Relu,1,2,698.5327659999999,110.91044283130478,1.5903890626017851,802816.0,11695808.0,133873664.0,dom
15,0,/features/features.21/Conv,1,2,758.7439659999999,120.47209048335807,1.3790918205953795,802816.0,14055104.0,131213312.0,dom
16,0,/features/features.25/Relu,1,2,758.5743339999999,118.18798686809288,1.3534044292920897,200704.0,16414400.0,128552960.0,dom
17,0,/features/features.27/Relu,1,2,763.305214,118.84419045282769,1.3286564625850343,200704.0,18773696.0,126193664.0,dom
18,0,/features/features.28/Conv,1,2,768.0360939999999,119.50039403756249,1.3047973117417564,200704.0,21132992.0,123759104.0,dom
19,0,/classifier/classifier.1/Relu,1,2,766.4693739999999,118.56036203756248,1.3047973117417564,8192.0,123893440.0,20881408.0,dom
20,0,/classifier/classifier.6/Gemm,1,2,766.4190059999999,118.53014123756249,1.3047973117417564,2000.0,144766656.0,1000.0,dom
21,0,/features/features.10/Conv,1,2,494.327374,92.29189921630368,3.429423022896474,1605632.0,6977216.0,139395072.0,dom
22,0,/features/features.12/Conv,1,2,554.538574,96.38357606922763,2.5777702988068842,1605632.0,7567040.0,138805248.0,dom
23,0,/features/features.16/MaxPool,1,2,604.948958,94.59476332215156,2.064963418760044,401408.0,8156864.0,137412608.0,dom
24,0,/features/features.17/Conv,1,2,638.321566,101.34879517925148,1.878149280713901,802816.0,9336512.0,136232960.0,dom
25,0,/features/features.19/Conv,1,2,698.5327659999999,110.91044283130478,1.5903890626017851,802816.0,11695808.0,133873664.0,dom
26,0,/features/features.24/Conv,1,2,758.5743339999999,118.18798686809288,1.3534044292920897,200704.0,16414400.0,128552960.0,dom
27,0,/features/features.26/Conv,1,2,763.305214,118.84419045282769,1.3286564625850343,200704.0,18773696.0,126193664.0,dom
28,0,/Flatten,1,2,766.8110699999999,118.76537963756249,1.3047973117417564,50176.0,21132992.0,123641856.0,dom
29,0,/classifier/classifier.0/Gemm,1,2,766.4693739999999,118.56036203756248,1.3047973117417564,8192.0,123893440.0,20881408.0,dom
30,0,/classifier/classifier.4/Relu,1,2,766.4693739999999,118.56036203756248,1.3047973117417564,8192.0,140670656.0,4098000.0,dom


==> figures/eyeriss_simba_efficient_UCIe_all_accuracy.tex <==
1,input,0.7557373,122.6137,86.1509,11.6075,8.16,edge
5,Mul_1,0.76123047,133.9885,86.589,11.5488,21.95,nondom
6,Mul_3,0.7565918,133.9885,86.589,11.5488,21.95,dom
9,Mul_4,0.76416016,136.8987,86.7531,11.527,64.59,opt
11,Mul_5,0.7553711,143.7854,87.4376,11.4367,16.77,dom
12,Mul_7,0.76501465,143.7854,87.4376,11.4367,16.77,nondom
18,Mul_13,0.75720215,174.8088,91.1288,10.9735,6.91,dom
19,Mul_15,0.75927734,174.8088,91.1288,10.9735,6.91,nondom
25,Mul_21,0.7680664,217.2217,97.1377,10.2947,3.17,dom
26,Mul_23,0.7680664,217.2217,97.1377,10.2947,3.17,opt2
28,Add_2,0.76660156,217.5702,97.2218,10.2858,1.06,nondom
33,Mul_33,0.7541504,267.7073,90.9254,10.998,5.42,dom
34,Mul_35,0.76013184,267.7073,90.9254,10.998,5.42,nondom
36,Add_4,0.7573242,268.5904,91.086,10.9786,1.76,dom
41,Mul_45,0.76220703,409.1273,99.099,10.0909,2.74,nondom
42,Mul_47,0.75756836,409.1273,99.099,10.0909,2.74,dom
45,Add_7,0.755249,468.2327,112.3476,8.9009,1.44,dom
50,Mul_61,0.76208496,559.9332,113.6801,8.7966,1.79,dom
51,Mul_63,0.7618408,559.9332,113.6801,8.7966,1.79,nondom
57,output,0.7624512,561.1936,113.855,8.7831,1.78,sensor

==> figures/partitioning.tex <==
\begin{figure}[t]
    \centering
    \scalebox{0.535}{
    \begin{tikzpicture}[
            > = stealth, % arrow head style
            shorten > = 1pt, % don't touch arrow head to node
            auto,
            node distance = 2cm, % distance between nodes
            semithick, % line style
            every node/.style = {font=\huge}
        ]

        \tikzstyle{every state}=[
            draw = KITgreen_70,
            thick,
            fill = KITgreen_30
        ]
        \tikzstyle{nstate}=[
            state,
            draw = KITred_70,
            fill = KITred_30,
        ]

        \node[]         (in)                        {\textbf{In}};
        \node[state]    (l1)  [right of=in]         {$l_1$};
        \node[nstate]   (l2)  [below right of=l1, xshift=1cm]   {$l_2$};
        \node[nstate]   (l3)  [above right of=l1]   {$l_3$};
        \node[nstate]   (l4)  [right of=l3]         {$l_4$};
        \node[state]    (l5)  [below right of=l4]   {$l_5$};
        \node[nstate]   (l6)  [right of=l5]         {$l_6$};
        \node[state]    (l7)  [right of=l6]         {$l_7$};
        \node[state]    (l8)  [right of=l7]         {$l_8$};
        \node[]         (out) [right of=l8]         {\textbf{Out}};

        
        \node[state, scale=0.6] (g) [below right of=l6, yshift=-1.5cm] {};
        \node[] [right of=g, xshift=-1.7cm, anchor=west]{\large{Potential Partitioning Point}};
        \node[nstate, scale=0.6] (r) [below of=g, yshift=0.8cm] {};
        \node[] [right of=r, xshift=-1.7cm, anchor=west]{\large{Not allowed}};

        \path[->] (in) edge                 (l1);
        \path[->] (l1) edge                 (l2);
        \path[->] (l1) edge                 (l3);
        \path[->] (l2) edge                 (l5);
        \path[->] (l3) edge                 (l4);
        \path[->] (l4) edge                 (l5);
        \path[->] (l5) edge                 (l6);
        \path[->] (l5) edge [bend left=60]  (l7);
        \path[->] (l6) edge                 (l7);
        \path[->] (l7) edge                 (l8);
        \path[->] (l8) edge                 (out);

        \node[rotate=90] (cut1) at (2.7, -2.4)  {\faCut};
        \node[KITgreen_100] (cut1_ok) at ([yshift=-0.2cm] cut1.west)  {\faCheck};
        \draw[black, dashed, thick] (2.7, 2.2) -- (cut1.center);
        
        \node[rotate=90] (cut2) at (5.7, -2.4)  {\faCut};
        \node[KITred_100] (cut2_ok) at ([yshift=-0.2cm] cut2.west)  {\faTimes};
        \draw[black, dashed, thick] (6.4, 2.2) -- (cut2.center);
        \draw[black, dashed, thick] (4.3, 2.2) -- (cut2.center);
    \end{tikzpicture}
    }
    \caption{Potential partitioning points within a DNN. $l_1$ is indicated as a suitable layer for segmentation without branching or redundant data transmissions. $l_2$ is highlighted as unsuitable because it is situated on a parallel branch.}
    \label{fig:partitioning}
\end{figure}
